Toeplitz Low-Rank Approximation with Sublinear Query Complexity

We present a sublinear query algorithm for outputting a near-optimal low-rank approximation to any positive semidefinite Toeplitz matrix $T \in \mathbb{R}^{d \times d}$. In particular, for any integer rank $k \leq d$ and $\epsilon,\delta > 0$, our algorithm makes $\tilde{O} \left (k^2 \cdot \log(1/\delta) \cdot \text{poly}(1/\epsilon) \right )$ queries to the entries of $T$ and outputs a rank $\tilde{O} \left (k \cdot \log(1/\delta)/\epsilon\right )$ matrix $\tilde{T} \in \mathbb{R}^{d \times d}$ such that $\| T - \tilde{T}\|_F \leq (1+\epsilon) \cdot \|T-T_k\|_F + \delta \|T\|_F$. Here, $\|\cdot\|_F$ is the Frobenius norm and $T_k$ is the optimal rank-$k$ approximation to $T$, given by projection onto its top $k$ eigenvectors. $\tilde{O}(\cdot)$ hides $\text{polylog}(d) $ factors. Our algorithm is \emph{structure-preserving}, in that the approximation $\tilde{T}$ is also Toeplitz. A key technical contribution is a proof that any positive semidefinite Toeplitz matrix in fact has a near-optimal low-rank approximation which is itself Toeplitz. Surprisingly, this basic existence result was not previously known. Building on this result, along with the well-established off-grid Fourier structure of Toeplitz matrices [Cybenko'82], we show that Toeplitz $\tilde{T}$ with near optimal error can be recovered with a small number of random queries via a leverage-score-based off-grid sparse Fourier sampling scheme.

==> approx_algorithm_old.tex <==
% !TEX root = ./main.tex

\section{Low-Rank Approximation with Sublinear Query Complexity}\label{algorithm}
%Now that we have established the existence of a good low rank approximation $\wt{T}$ which itself is Toeplitz, we present an alg orithm that constructs such a low rank approximation by only reading $poly(k)<<d$ entries of $T$. Note that we can trivially recover $T$ exactly by reading all the entries of the first column, that is the trivial sample complexity for this problem is $d$ samples. \\
In this section, we present our main algorithm, Algorithm \ref{sublinearqueryalgo} and prove the corresponding Theorem \ref{sublinearqueryalgo}, which shows that the algorithm outputs a near optimal low-rank approximation to $T$, while reading only sublinearly many entries. 
We treat $\wt{T}$, the low-rank Toeplitz approximation to $T$ (guaranteed to exist from Theorem \ref{frobeniusexistence}), as the true matrix, which we noisily access by reading entries of $T$.

\subsection{Main algorithm}

%\hltodo{Need to double check the sparsity is updated throughout this section for the $1+\epsilon$ approximation: $\wt{O}(\frac{k}{\epsilon}\log(\frac{1}{\delta}))$} 
The near optimal Toeplitz low-rank approximation $\wt T \in \R^{d \times d}$ guaranteed to exist by Theorem \ref{frobeniusexistence} is of the form $\wt T =F_{\wt{S}}\wt{D}F_{\wt{S}}^{*}$, where $ F_{\wt{S}}\in \mathbb{C}^{d\times r}$ and $\wt{D}\in \mathbb{R}^{\wt{O}(r\times r}$ are Fourier and diagonal matrices, respectively, and $r=\wt{O}(\frac{k}{\epsilon}\log(1/\delta))$. At a high level, Algorithm \ref{sublinearqueryalgo} uses brute force search to find the frequencies in $\wt{S}$. In particular, it uses an approximate regression oracle to test the quality of any guess for the frequencies in $\wt{S}$, without reading many entries of $T$.  

\hltodo{Need to double check the sparsity is updated throughout this section for the $1+\epsilon$ approximation: $\wt{O}(\frac{k}{\epsilon}\log(\frac{1}{\delta}))$} 
The near optimal Toeplitz low-rank approximation $\wt T \in \R^{d \times d}$ guaranteed to exist by Theorem \ref{frobeniusexistence} is of the form $\wt T =F_{\wt{S}}\wt{D}F_{\wt{S}}^{*}$, where $ F_{\wt{S}}\in \mathbb{C}^{d\times \wt{O}(\frac{k}{\epsilon}\log(1/\delta))}$ and $\wt{D}\in \mathbb{R}^{\wt{O}(\frac{k}{\epsilon}\log(1/\delta))\times \wt{O}(\frac{k}{\epsilon}\log(1/\delta))}$ are Fourier and diagonal weight matrices, respectively. At a high level, Algorithm \ref{sublinearqueryalgo} uses brute force search to find the frequencies in $\wt{S}$. In particular, it uses an approximate regression oracle to test the quality of any guess for the frequencies in $\wt{S}$, without reading many entries of $T$.  

Recall from Theorem \ref{frobeniusexistence} that these frequencies lie in $r_1 = \tilde O(k/\epsilon)$  clusters of equispaced frequencies centered around points in $N =\{1/2d,3/2d,\ldots, 1-1/2d\}$. Thus, our search space will be all subsets of $r_1$ elements of $N$, of which there at at most $N^{r_1}$. Since the first column of $\wt{T}$ defines $\wt{T}$, the approximate regression oracle will simply attempt to fit the first column of $\wt{T}$. However, since different entries in the first column of $\wt{T}$ appear with different frequencies in $\wt{T}$, we require the following weighting function to translate error bounds in the first column into error bounds for approximating the entire matrix $\wt{T}$ in the Frobenius norm. 
\begin{definition}\label{weightingdef}
	Let $w\in \mathbb{R}^{d}$ be defined as follows:
	\begin{equation*}
		w_{i} =  \begin{cases} 
			\sqrt{d} & i = 1 \\
			\sqrt{2(d-i+1)} & i > 1 
		\end{cases}
	\end{equation*}
	Let $W = \diag(w)\in \mathbb{R}^{d\times d}$.
\end{definition}
We have the following immediate claim, which expresses the Frobenius norm of a symmetric Toeplitz matrix as the weighted $\ell_2$ norm of its first column. 
\begin{claim}\label{frobtoeuclid}
	Let $T\in \mathbb{R}^{d\times d}$ be a symmetric Toeplitz matrix and let $T_{1}\in \mathbb{R}^{d}$ be its first column. Then $\|T\|_F = \|WT_1\|_2$, where $W$ is as in Definition \ref{weightingdef}.
\end{claim}
%While performing the brute force search over all possible frequencies, we need an approximate regression oracle which accesses only a few rows of the coefficient matrix ($F_S$) and entries of the label vector ($T_1$), and evaluates how well those frequencies fit the samples of $T$. We can achieve this using leverage score sampling, which requires bounding the sum of leverage scores of our coefficent matrix (a weighted Fourier matrix). We recall the definition of leverage scores (\ref{leveragescoresdefn}) as introduced in \cref{sec:preliminaries}.

\medskip

\noindent\textbf{Leverage Score Sampling.} 
To perform the brute force search over all possible frequency sets $\tilde S$, we need an approximate regression oracle, which accesses only a few entries of $T_1$. We will construct such an oracle using leverage score sampling. The \emph{leverage scores} \cite{spielman2011graph,drineas2006sampling} of a matrix are formally defined in \cref{leveragescoresdefn} below.
\begin{definition}\label{leveragescoresdefn}
	For any $A\in \mathbb{C}^{d\times r}$ and $j\in [d]$ let $\tau_j(A)$ denote the leverage score of the $j^{th}$ row of $A$:
	\begin{equation}
		\tau_j(A) = \max_{y\in \mathbb{C}^{s}} \frac{|(Ay)_i|^2}{\sum_{j=1}^d |(Ay)_j|^2}.
	\end{equation}
\end{definition}
It is known that leverage score sampling can be used to approximately solve linear regression problems in a sample-efficient manner. We will use  \cref{thm:updatedleveragesampling}, which formalizes this.  \cref{thm:updatedleveragesampling} gives worse $\epsilon$ and log dependencies than standard results on approximate regression with leverage score sampling \cite{Sarlos:2006vn,Woodruff:2014tg}. However, it provides two key guarantees that such theorems do not: 1) it gives a logarithmic dependence on the failure probability, which will be key in our setting, since we need to take a union bound over $N^{r_1}$ regression problems, and 2) it gives an estimate to the error of the approximate regression solution, which will be critical in choosing the set $\wt S$ that gives $\wt T$ best fitting $T$.
\iffalse
one can obtain spectral approximations to matrices by sampling their rows using probabilities proportional to their leverage scores. The following lemma formalizes this for complex matrices. 
\begin{lemma}[Corollary 5.2 in \cite{tropp2012user}]\label{leveragescoresampling}
	\hltodo{Do we still need this lemma? Check back}
	\mmtodoil{corollary 5.2 is matrix Chernoff, this lemma is considerably different to warrant some explanations how we get it from there.\\
	Is the first claim really true? I would personally expect that it holds with high probabilty for each $x$, not for all of them. }
	Given a matrix $A\in \mathbb{C}^{d\times r}$ and values $\wt{\tau}_{1},\ldots,\wt{\tau}_{d}\in [0,1]$ that satisfy the following for all $j\in [n]$.
	\begin{equation*}
		\wt{\tau}_{j}\geq \tau_{j}(A) 
	\end{equation*}
	Then there are universal constants $c,C$ such that if we perform the following:
	\begin{enumerate}
		\item Set $p_{j}= \min (1,c\wt{\tau}_{j}\log(r/\delta_{1})/\epsilon^2)$.
		\item Create a sampling matrix $P\in \mathbb{C}^{s\times d}$ that takes $s$ samples as follows - Sample each row $a_j$ of $A$ independently with probability $p_j$ and add a row with $1/\sqrt{p_j}$ at the $j^{th}$ entry and $0$ elsewhere to $P$ for each such sampled row $a_j$. 
	\end{enumerate}
	Then the following holds with probability at least $1-\delta_{1}$:
	\begin{enumerate}
		\item $(1-\epsilon)\|Ax\|_2^2\leq \|PAx\|_2^2\leq (1+\epsilon)\|Ax\|_2^2$ for all $x\in \mathbb{C}^{d}$.
		\item $s\leq \frac{C\log(r/\delta_1)}{\epsilon^2}\sum_{j=1}^{d}\wt{\tau}_{j}$.
	\end{enumerate}
\end{lemma}
\fi
First, we need to formally define leverage score \emph{sampling} below.
\begin{definition}[Leverage score sampling; Def. 2.7 of \cite{musco2021active}]\label{def:levsampling}
	For any number of samples $m$ and a set of leverage score bounds $\{\tilde \tau_j \}_{j \in [n]}$ (which upper bound the true leverage scores $\tau_j$ of some matrix with $d > m$ rows) with $T = \sum_{j=1}^d \wt{\tau}_j$, let $\mathcal{S} \in \mathbb{R}^{m \times d}$ be a sampling matrix with each row set independently to the $i^{th}$ standard basis vector multiplied by $(m \cdot p_i)^{-1/2}$, with probability 
	\begin{align*}
		p_i &= \frac{1}{2} \Bigg( \frac{\wt{\tau}_i}{T} + \frac{1}{d} \Bigg).
	\end{align*}
\end{definition}

Using \cref{def:levsampling}, we are ready to state \cref{thm:updatedleveragesampling}. 
\begin{theorem}[High-probability $(1+\epsilon)$-regression using leverage scores]\label{thm:updatedleveragesampling}
Suppose we are given $A \in \mathbb{R}^{d \times r}$, query access to $b \in \mathbb{R}^d$, an accuracy parameter $\epsilon>0$, failure probability $\eta>0$, and leverage score upper bounds  $\wt{\tau}_j$ that satisfy $\wt{\tau}_j \ge \tau_j(A)$ for all $j \in [n]$. Suppose further that $\sum_j\wt{\tau}_j = T$. 

Let $\mathcal{S} \in \mathbb{R}^{m \times d}$ be a random sampling matrix drawn according to \cref{def:levsampling}, using the distribution $\wt{\tau}_j$ and $m=O\big(\frac{T \log^2(T) \log(1/\eta)}{\epsilon^9}\big)$ samples. Then there is an algorithm \texttt{LevSample}($\mathcal{S}A$, $\mathcal{S}b$, $\epsilon$, $\eta$) outputting with probability $1-\eta$ over the randomness of $S$,
\begin{enumerate}
\item $\wt{x} \in \R^d$ satisfying $\|A\wt{x}-b\|_2 \leq (1+\epsilon)\min_{x \in \mathbb{R}^r}\|Ax-b\|$.
\item An approximate cost $val(\wt x) \in \R$ satisfying $|val(\wt x) - \|A\wt{x}-b\|_2 - C | \le \epsilon \cdot  \|A\wt{x}-b\|_2$ where $C$ is a constant that depends only on the leverage score upper bounds $\{\tilde \tau_j \}_{j \in [n]}$ and $b$.
\end{enumerate}
\end{theorem}
\begin{proof}
\Cam{Cameron will do later tonight.}
This theorem follows\footnote{Although the original theorem statement from \cite{musco2021active} assumes access to the exact leverage scores, all proofs go through using only leverage score \emph{upper bounds} as well.} by combining Theorem 3.4 and Section 4 of \cite{musco2021active} for the $\ell_2$ norm, i.e. $p=2$.
\end{proof}

\iffalse
We will need one more result from \cite{musco2021active} to enable our sublinear sample complexity algorithm. In the notation of \cref{thm:updatedleveragesampling}, after sampling by leverage scores, we also need the sampled error estimate of the computed coefficients $\|\mathcal{S}A\tilde{x}-\mathcal{S}b\|_2$ to capture well the true error $\|A\tilde{x}-b\|_2$. The following theorem shows that this will hold up to a constant offset.

\begin{theorem}\label{thm:leverage_score_error}
	In the setting of \cref{thm:updatedleveragesampling}, $\tilde{x}$ satisfies the following inequality:
	\begin{align*}
		\| \|\mathcal{S}A\tilde{x}-\Sb\|_2 - \|A\tilde{x}-b\|_2 \| = 
	\end{align*}
\end{theorem}

This theorem follows from Lemma 3.7 and the proof of Theorem 3.4 in \cite{musco2021active}.
\fi 

Let $F_S \in \mathbb{C}^{d \times r}$ be a symmetric Fourier matrix corresponding to some frequencies $S=\{f_1,\dots,f_{r/2}\} \subset [0,1]$ as in \cref{def:symmetric_fourier_matrix}. In our setting, we will obtain non-trivial leverage score upper bounds on $WF_S$, which are crucially \emph{universal} (in the sense that they are independent of $S$). The importance of having \emph{universal} leverage score bounds is that a single set of samples will work for \emph{all} possible guesses of the true frequencies $\tilde{S}$ in our brute force search. However, note that \cref{thm:updatedleveragesampling} applies only to \emph{real} matrices as stated. In the notation of \cref{thm:updatedleveragesampling}, although we are sampling a real-valued vector $b$ (corresponding to the weighted first column of $T$) and seeking a real-valued vector $x$, the regression matrix itself is complex, $A=WF_S$. This is possible only because we would like to require that $x$ takes equal values at indices corresponding to symmetric frequencies (in the sense of \cref{thm:vandermonde}). To incorporate both this restriction on $x$ and the real-valued requirement of \cref{thm:updatedleveragesampling}, we introduce a new frequency-dependent matrix, $R_S$, which collapses the $2|S|=r$ conjugate pair columns of $WF_S$ into $|S|=\frac{r}{2}$ real-valued columns, each corresponding to a degree of freedom of $x$. %\Cam{Like in Def 1.2 we need to result the issues of odd $r$ here.}

\begin{definition}\label{def:RS} 
Let $S \subset [0,\frac{1}{2})$ with $|S|=\frac{r}{2}$. % with $|S| = \frac{r}{2}$. 
Then, define the matrix $R_S \in \mathbb{R}^{2|S| \times |S|}$ (or equivalently $R_S \in \mathbb{R}^{r \times \frac{r}{2}}$) by setting the $j^{th}$ column $(R_S)_{:,j}$ equal to $0$ everywhere except at $j$ and $|S|+j$, corresponding to the $j^{th}$ \emph{pair} of conjugate frequencies, where it is equal to $1$. %(Here, we assume that both $S$ and the frequency pairs are ordered according to some arbitrary ordering.)  
%\Cam{Fix to match new notation later.}\hltodo{Checking back, it seems like $r$ is indeed used as the rank and $F_S$, $F_{-S}$ are ordered correspondingly? What exactly needs to be changed (or what earlier sec. has the inconsistency)?}
\end{definition}
%Note in the above definition that if $r$, the rank of a Toeplitz matrix, is odd, then there exists some frequency in its Vandermonde decomposition which is its own conjugate. According to the convention of \cref{def:symmetric_fourier_matrix}, the frequency set $S$ is then of size $\frac{r}{2} \rceil$, where the column vector of $F_S$ corresponding to the self-conjugate frequency is repeated. This motivates the dimensionality of $R_S$ in the case when $r$ is odd. 

It is trivial to check from this definition that $F_SR_S$ is always real-valued, so we can equivalently interpret $F_S$ applied to any $r$-length symmetric vector $x$ (which takes equal values on conjugate frequencies, ie. $x_j=x_{\frac{r}{2}+j}$ for $j\in[\frac{r}{2}]$) as $F_SR_S$ applied to the $\frac{r}{2}$-length scaled subset of $x$, $\frac{1}{2}R_S^Tx$. Therefore, we will apply leverage score sampling to the real-valued matrix $F_SR_S$, and optimize only over the desired $\frac{r}{2}$ degrees of freedom.

To apply \cref{thm:updatedleveragesampling} in the proof of our approximate regression oracle, we therefore need good upper bounds on the leverage scores of $WF_SR_S$. We obtain such bounds in this section, which are in fact independent of the frequencies $S$. This is formalized in the following lemma.
\begin{lemma}\label{leveragescorebound}
	Let $W$ be the weight matrix defined in \cref{weightingdef}. Then there exist non-negative numbers $\{\wt{\tau}_{j}\}_{j=1}^d$ such that the following hold for all frequency sets $S\subset [0,\frac{1}{2}), |S| = \frac{r}{2}\leq d$: 
	\begin{enumerate}
		\item $\tau_j(WF_SR_S) \leq \tau_j(WF_S) \leq \wt{\tau}_{j}$ for all $j\in [d]$.
		\item $\sum_{j=1}^{d} \wt{\tau}_{j} \leq O(r\log (d)\log (r))$.
	\end{enumerate}
	Here, $F_S\in \mathbb{C}^{d\times r}$ is the symmetric Fourier matrix with frequency set $S$ as defined in \cref{def:symmetric_fourier_matrix}, and $R_S$ is as defined in \cref{def:RS}. 

\end{lemma}
\cref{leveragescorebound} is similar to Corollary C.2 of \cite{eldar2020toeplitz}, but applies to \emph{weighted} Fourier matrices. (Corollary C.2 of \cite{eldar2020toeplitz} holds only for $W=I$, and does not have the $\log(d)$ dependence in the upper bound on $\sum_{j=1}^{d} \wt{\tau}_{j} $.) We will later restate Corollary C.2 of \cite{eldar2020toeplitz} as \cref{corr:C2_eldar}, and use it in the proof of \cref{leveragescorebound}, which we defer to \cref{subsec:weighted_fourier_lev_bounds}.

Equipped with these tools, we now describe the recovery algorithm and its guarantees. %The proofs of the previous lemmas are presented in the next sub-section after the proof of correctness of the algorithm.

\begin{algorithm}[H] 
	\SetAlgoLined
	$\textbf{Input:}$ Query access to $T\in \mathbb{R}^{d\times d}$, $k, \epsilon, \delta,\gamma$\; 
	$\textbf{Init:}$ Set $N=\{\frac{1}{2d},\frac{3}{2d},\ldots, 1-\frac{1}{2d}\}$, $r_1=O(k\log^8d/\eps)$, $r_2 = O(\log d +\log(1/\delta))$, $\eta=\frac{1}{100|N|^{r_1}}$ \; %\Cam{Make sure $r_1$ and $r_2$ exactly match valued defined in Thm 4, which I think have changed a little (and which I've suggested more changes to).}
	Set $F = [0]_{d\times r_1r_2}$, $d = [0]_{r_1r_2\times 1}$ and $OPT=0$\;
	%Let $P\in \mathbb{R}^{s\times d}$ be an i.i.d. sampling matrix as per Lemmas \ref{leveragescoresampling} and \ref{leveragescorebound} \;
	Draw $\mathcal{S}$ according to \cref{def:levsampling}, using $\wt{\tau}_j$ (from \cref{leveragescorebound}) with $m=\tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^{11}} \Big)$ %O\big(\frac{r\log^2(d)\log^3(r)\log(1/\delta)}{\epsilon^9}\big)$ 
	samples \\
	\For{all $B\in N^{r_1}$}{
		For all $f_i\in B$ define $B_i$ as follows:
		\begin{equation*}
			B_i = \underset{1\leq j\leq r_2}{\bigcup}\{f_i+\gamma j,f_i-\gamma j\} %,-(f_i+\gamma j),-(f_i-\gamma j)\}
		\end{equation*}
		Let $F_{S(B)}$ be the symmetric Fourier matrix corresponding to $S(B)=\underset{1\leq i\leq r_1}{\bigcup}B_i$\;
		
		Let $val(d_{S(B)}), \: d_{S(B)} = \texttt{LevSample}(\mathcal{S}WF_{S(B)}R_{S(B)}, \mathcal{S}WT_1, \epsilon, \eta)$ %, and $val(d_{S(B)}) = \|\mathcal{S}WF_{S(B)}R_{S(B)}d_{S(B)}-\mathcal{S}WT_1\|_2$ 

		%Let $d_{S(B)} = \argmin_{x}\|PWF_{S(B)}x-PWT_1\|_2 $ and $val(d_{S(B)}) =\min_{x}\|PWF_{S(B)}x-PWT_1\|_2  $\;

		\textbf{If} $val(d_{S(B)})\leq OPT$ \textbf{then} $OPT = val(d_{S(B)}),F = F_{S(B)},d = R_{S(B)}d_{S(B)}$\;
	}
	
	$\textbf{Return:}$ $F,d$
	\caption{\textsc{ToeplitzRecovery}}\label{toeplitzrecovery}
\end{algorithm}
\begin{theorem}\label{sublinearqueryalgo}
	Assume we are given query access to a PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$ and parameters $k,\delta$. Let  $r = r_1r_2 = \wt{O}(\frac{k}{\epsilon}\log(1/\delta))$. Then Algorithm \ref{toeplitzrecovery} returns $F\in \mathbb{C}^{d\times r},d\in \mathbb{R}^{r}$ such that $F \diag(d)F^{*}$ is a symmetric Toeplitz matrix of rank $O(r)$\hltodo{I added big O here - it's not exactly r} and the following holds.
	\begin{enumerate}
		\item Algorithm \ref{toeplitzrecovery} makes $\tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^{11}} \Big)$ %$O\big(\frac{r\log(d)\log^2(r) \log^2(r\log(d)\log(r)) \log(1/\delta)}{\epsilon^9}\big)$ %$\wt{O}(k^2\log(1/\delta))$
		 queries to $T$. 
		\item $\|T-F\diag(d)F^{*}\|_F\leq (1+\epsilon)^2\|T-T_k\|_F + \delta(1+\epsilon) \|T\|_F$ with probability at least $99/100$. \hltodo{This guarantee needs to be updated and epsilon/delta modified based on the final guarantee}
	\end{enumerate}
\end{theorem}
\begin{proof}
	
	Let $F_{\wt{S}},\wt{D}$ be the Fourier and diagonal matrices guaranteed to exist by Theorem \ref{frobeniusexistence}, and recall that $F$ and $d$ are the Fourier matrix and vector, respectively, returned by Algorithm \ref{toeplitzrecovery}.  Let $B',d' = \underset{B\in N^{r_1},x\in \mathbb{R}^{r}}{\argmin} \|W(F_{S(B)}x-T_1)\|_2$ and $F'=F_{S(B')}$. Since Algorithm \ref{toeplitzrecovery} brute force searches over all possible frequencies having the structure described in part \ref{thm:existence_freq_grid} of Theorem \ref{frobeniusexistence}, and uses the same $\gamma$ as per Theorem \ref{frobeniusexistence}, by Claim \ref{frobtoeuclid} we have the following:
	\begin{align*}
		\|WF'd'-WT_1\|_2&=\underset{B\in N^{r_1},x\in \mathbb{R}^{\frac{r}{2}}}{\min} \|W(F_{S(B)}x-T_1)\|_2 \\&= \underset{B\in N^{r_1},x\in \mathbb{R}^{\frac{r}{2}}}{\min} \|F_{S(B)}\diag(x) F_{S(B)}^{*}-T\|_F\\
		&\leq \|F_{\wt{S}}\wt{D}F_{\wt{S}}-T\|_F\\
		&\leq (1+\epsilon)\|T-T_k\|_F + \delta \|T\|_F.
	\end{align*}
	We then apply \cref{thm:updatedleveragesampling} with $\epsilon=\epsilon$, $\eta = \frac{1}{100|N|^{r_1}}$, and the upper bounds $\wt{\tau}_j$ are as described in \cref{leveragescorebound}, and crucially use the \emph{same} samples every time \texttt{LevSample} is called. Since the probability of failure each time \texttt{LevSample} is called is at most $\eta = \frac{1}{100|N|^{r_1}}$, and \texttt{LevSample} is called $|N|^{r_1}$ times, via a union bound the probability that any one of the calls fails is at most $\frac{1}{100}$. Therefore, with probability at least $\frac{99}{100}$, every call to $\texttt{LevSample}$ returns a $(1+\epsilon)$-approximation and a validation error satisfying (2) of \cref{thm:updatedleveragesampling}. When this occurs, then we can upper bound the error $||F\diag(d)F^*-T||_F = ||WFd - WT_1||_2$ of the returned matrix as follows.

	First, by part (2) of \cref{thm:updatedleveragesampling}, observe that $val(d)$ is within $\epsilon\|WFd-WT_1\|_2$ of $\| WFd-WT_1\|_2 + C$, and likewise for $val(d')$:
	\begin{align*}
		|val(d) - (\| WFd-WT_1\|_2 + C)| &\leq \epsilon\|WFd-WT_1\|_2 \\
		|val(d') - (\| WF'd'-WT_1\|_2 + C)| &\leq \epsilon\|WF'd'-WT_1\|_2.
	\end{align*}
	Moreover, by design of Algorithm \ref{algorithm}, $val(d) \leq val(d')$. Therefore, $\|WFd-WT_1\|_2$ and $\|WF'd'-WT_1\|_2$ are within at most $\epsilon(\|WFd-WT_1\|_2 + \|WF'd'-WT_1\|_2)$ of one another, as shown below.
	\begin{align*}
		\|WFd-WT_1\|_2 - \|WF'd'-WT_1\|_2 &= (\|WFd-WT_1\|_2 + C) - (\|WF'd'-WT_1\|_2 + C) \\
		&\leq (val(d) + \epsilon\|WFd-WT_1\|_2) - (val(d') -  \epsilon\|WF'd'-WT_1\|_2) \\
		&= (val(d) - val(d')) + \epsilon(\|WFd-WT_1\|_2 + \|WF'd'-WT_1\|_2) \\
		&\leq \epsilon(\|WFd-WT_1\|_2 + \|WF'd'-WT_1\|_2) 
	\end{align*}
	Rearranging terms and applying the previous bound on $\|WF'd'-WT_1\|_2$ then yields
	\begin{align*}
		\|WFd-WT_1\|_2 \leq \frac{1+\epsilon}{1-\epsilon} \|WF'd'-WT_1\|_2 \\
		\leq \frac{(1+\epsilon)^2}{1-\epsilon}\|T-T_k\|_F + \frac{\delta(1+\epsilon)}{1-\epsilon} \|T\|_F\\
	\end{align*}
 
	\iffalse
	\begin{align*}
		\|WFd - WT_1\|_2 &\leq (1+\epsilon) \min_{B\in N^{r_1}, x \in \mathbb{R}^{\frac{r}{2}}}\|WF_{S(B)}x-WT_1\|_2 \\  
		&\leq (1+\epsilon)^2 ||T-T_k|| + \delta (1+\epsilon)||T||_F
	\end{align*}
	The first inequality above followed by the guarantee of \cref{thm:updatedleveragesampling} combined with the optimality of $F$ and $d$, while the second inequality follows from the earlier bound on $\|WF'd'-WT_1\|_2$. 
	\fi

	Substituting $T = O(r\log(d)\log(r))$ into the guarantee of \cref{thm:updatedleveragesampling} yields $m=\tilde{O}\big(\frac{r\log^3(r)\log(1/\eta)}{\epsilon^{9}}\big)$, where $r=\tilde{O}(\frac{k \log(1/\delta)}{\epsilon})$ from \cref{sec:existence_main}, $|N| = O(d)$, $\eta = \frac{1}{100|N|^{r_1}}$, and $\tilde{O}$ notation hides $\log(d)$ factors. Further simplifying this expression completes the proof of the sample complexity of Algorithm \ref{toeplitzrecovery}.\hltodo{Use different $\epsilon$ for lev score and rest of paper so that the final guarantee is cleaner}

	% below: the old proof (constant factor approx)

	\hltodoil{Old proof below, uncommenting}

	We can write $\|WFd - WF'd'\|_2$ as $\|W[F;F']([d^{T};{d'}^{T}])^{T}\|_2$. Here $[F;F']\in \mathbb{C}^{d\times 2r}$ is also a Fourier matrix. We apply Lemma \ref{leveragescoresampling} with $\epsilon=9$, $\delta_{1} = 1/(100|N|^{r_1})$, and $\wt{\tau}_j$ values for $d\times 2r$ dimensional weighted Fourier matrices as per Lemma \ref{leveragescorebound} to obtain a sampling matrix $P\in \mathbb{R}^{s\times d}$ that takes $s=O(\log(d|N|^{r_1}) 2r \log (d)\log (r)) = \wt{O}(k^2\log(1/\delta))$ samples. Taking a union bound over all $B\in N^{r_1}$ we get the following which holds with probability at least $1-|N|^{r_1}\delta_1 = 99/100$ over the choice of $P$.
	\begin{align*}
		\|PW[F_{S(B)};F']x\|_2 \leq 10 \|W[F_{S(B)};F']x\|_2 \quad \forall B\in N^{r_1}, x\in \mathbb{C}^{2r}
	\end{align*}
	This in particular implies that  the following holds with probability at least $99/100$.
	\begin{align*}
		\|WFd - WF'd'\|_2 &\leq 10 \|PWFd - PWF'd'\|_2\\
		&\leq 10 (\|PWFd - PWT_1\|_2 + \|PWF'd' - PWT_1\|_2)\\
		&\leq 10 (\|PWF'd' - PWT_1\|_2 + \|PWF'd' - PWT_1\|_2)\\
		&= 20\|PWF'd'-PWT_1\|_2
	\end{align*}
	Where the third inequality follows by observing that $F,d = \underset{B\in N^{r_1},x\in \mathbb{R}^{r}}{\argmin} \|PWF_{S(B)}x-PWT_1\|_2$. Now by the unbiasedness property of the sampling matrix $P$ as per Lemma \ref{leveragescoresampling} we get that $\mathbb{E}[\|PWF'd'-PWT_1\|_2^2] = \|WF'd'-WT_1\|_2^2$. Thus applying Markov's inequality we get that $\|PWF'd'-PWT_1\|_2\leq 10 \|WF'd'-WT_1\|_2$ with probability $99/100$. Thus taking a union bound we get that the following holds with probabililty at least $98/100$ over the choice of $P$.
	\begin{align*}
		\|WFd - WT_1\|_2 &\leq \|WF'd'-WT_1\|_2 + \|WFd - WF'd'\|_2	\\		
		&\leq \|WF'd'-WT_1\|_2 +  20\|PWF'd'-PWT_1\|_2\\
		& \leq \|WF'd'-WT_1\|_2 +  200\|WF'd'-WT_1\|_2 \\
		& \leq 201\|WF'd'-WT_1\|_2\\
		& \leq \wt{O}(1)\|T-T_k\|_F + \delta \|T\|_F
	\end{align*}
	Thus we can finally conclude the following which completes the proof of point 2 of the theorem.
	\begin{equation*}
		\|F\diag(d)F^{*}-T\|_F = \|WFd - WT_1\|_2 \leq \wt{O}(1)\|T-T_k\|_F + \delta \|T\|_F
	\end{equation*}
	Note that while computing $d_{S(B)} = \argmin_{x}\|PWF_{S(B)} - PWT_1\|_2$ for any $B\in N^{r_1}$ we can restrict $x$ to have the same value for any frequency and its negative counterpart. This would ensure that $ F_{S(B)}\diag(d_{S(B)})F_{S(B)}^{*}$ is a real symmetric Toeplitz matrix for any $B\in N^{r_1}$. The proof above goes through even with this modification. Finally, we only need to know $PWT_1$ while executing our algorithm. This requires reading just $s=\wt{O}(k^2\log(1/\delta))$ entries of $T_1$, as specified by the $s\times d$ sampling matrix $P$.

\end{proof}

\subsection{Leverage score bounds for weighted Fourier matrices}\label{subsec:weighted_fourier_lev_bounds}
In this subsection, we focus on proving the leverage score upper bounds for weighted Fourier matrices of Lemma \ref{leveragescorebound}. Recall the statement of Lemma \ref{leveragescorebound} was as follows.
\begin{replemma}{leveragescorebound}
	Let $F_S\in \mathbb{C}^{d\times r}$ be any Fourier matrix with symmetric (in the sense of \cref{thm:vandermonde}) frequency set $S\subset [0,1], |S| = r\leq d$,$r\leq d$, and let $W$ and $R_S$ be as defined in \cref{weightingdef} and \cref{def:RS}. Then there exist non-negative numbers $\wt{\tau}_{j}$ for all $j\in [d]$ such that the following hold:
	\begin{enumerate}
		\item $\tau_j(WF_SR_S) \leq \tau_j(WF_S) \leq \wt{\tau}_{j}$ for all $j\in [d]$.
		\item $\sum_{j=1}^{d} \wt{\tau}_{j} \leq O(r\log (d)\log (r))$.
	\end{enumerate}
\end{replemma}

To prove this lemma, we will use the following three helper lemmas. %Their proofs are deferred to the end of this subsection. \hltodo{Is it really easier to defer these proofs? The proof of lemma 4.4 is already out of order}
\begin{lemma}\label{levscore_reweight}
Let $A \in \mathbb{C}^{d \times r}$ be a matrix, and let $D$ be a diagonal matrix with positive entries satisfying %$$\max_{i,j}\frac{D_{jj}}{D_{ii}} \leq C $$
$$ \alpha \leq D_{ii}^2 \leq \beta $$
Then, 
$$ \tau_i(DA) \leq \frac{\beta}{\alpha}\tau_i(A) $$
\end{lemma}
%We now finish this subsection with the proofs of helper Lemmas \ref{levscore_reweight} and \ref{levscore_submatrix}respectively. 
\begin{proof}[Proof of Lemma \ref{levscore_reweight}]
	By the definition of leverage scores, we have the following:
	$$\tau_i(DA) = \max_{y\in \mathbb{C}^{r}} \frac{|DAy|_i^2}{\sum_{j=1}^d |DAy|_j^2} $$
	For any $y$, the numerator is given by $|DAy|_i^2 = D_{ii}^2|Ay|_i^2$. The denominator satisfies
	$$ \sum_{j=1}^d |DAy|_j^2 \geq \alpha \sum_{j=1}^d |Ay|_j^2$$
	As a result,
	$$ \max_{y\in \mathbb{C}^{r}} \frac{|DAy|_i^2}{\sum_{j=1}^d |DAy|_j^2} = \max_{y \in \mathbb{C}^{r}} \frac{D_{ii}^2|Ay|_i^2}{\sum_{j=1}^d |DAy|_j^2} \leq \max_{y\in \mathbb{C}^{r}} \frac{\beta|Ay|_i^2}{\alpha\sum_{j=1}^d |Ay|_j^2}$$
	This proves that $ \tau_i(DA) \leq \frac{\beta}{\alpha}\tau_i(A)$ as desired.
\end{proof}

\begin{lemma}\label{levscore_submatrix}
Let $A \in \mathbb{C}^{d \times r}$ be a matrix, and let $B \in \mathbb{C}^{d' \times r}$ be a matrix formed by taking any subset $R \subseteq [1,\dots,d]$ of the rows of $A$. Then the leverage score of any row $b_i$ in $B$ is at least the leverage score of row $b_i$ in $A$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{levscore_submatrix}]
	Let $b_i$ correspond to the $i^{th}$ row of $A$ and the $i'^{th}$ row of $B$. Then by the definition of leverage scores we have the following.
	\begin{align*}
		\tau_i(A) &= \max_{y} \frac{|Ay|_i^2}{\sum_{j=1}^d |Ay|_j^2} \\
		&\leq \max_{y} \frac{|Ay|_i^2}{\sum_{j \in R} |Ay|_j^2} \\
		&= \max_{y} \frac{|By|_{i'}^2}{\sum_{j=1}^{d'} |By|_j^2} \\
		&= \tau_{i'}(B)
	\end{align*}
	
\end{proof}
\begin{lemma}\label{lemma:lev_score_col_span}
	Let $A \in \mathbb{C}^{d \times r}$ be a matrix, and let $B \in \mathbb{C}^{d \times r'}$ be a matrix formed by taking $r'<r$ linear combinations of the columns of $A$ (i.e. there is some matrix $M \in \mathbb{C}^{r \times r'}$ such that $B = AM$). Then the $i^{th}$ leverage score of $B$, $\tau_i(B)$, is at most the $i^{th}$ leverage score of $A$, $\tau_i(A)$. 
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:lev_score_col_span}]
	We again rely on the maximization characterization of leverage scores: 
	\begin{align*}
		\tau_i(B) &= \max_{y} \frac{|By|_i^2}{\sum_{j=1}^d |By|_j^2} \\
		&= \max_{y} \frac{|AMy|_i^2}{\sum_{j=1}^d |AMy|_j^2} \\
		&\leq \max_{z} \frac{|Az|_i^2}{\sum_{j=1}^d |Az|_j^2} \\
		&= \tau_i(A)
	\end{align*}
	where the second inequality follows from the fact that $\{ My | y \in \mathbb{C}^{r'} \} \subseteq \{ z | z \in \mathbb{C}^r\}$.
\end{proof}
Equipped with these lemmas, the high level strategy for bounding the leverage scores of $WF_SR_S$ is as follows. By \cref{lemma:lev_score_col_span}, it suffices to bound the leverage scores of $WF_S$. To do so, first we will bucket the rows of $WF_S$ into submatrices, such that within each submatrix, the weights vary by at most a constant factor. We will then be able to bound the leverage scores of each submatrix using Lemma \ref{levscore_reweight}, and apply Lemma \ref{levscore_submatrix} to ensure that these upper bounds remain valid upper bounds for the entire matrix $WF_S$.

Formally, begin by dividing $WF_S$ into submatrices as follows.
\begin{definition}
For all $i\in [\log d]$, let $W_i$ %\in \mathbb{R}^{(d/2^{i})\times d}$ 
be the submatrix of $W$ consisting of rows with indices in $[d(1-1/2^{i-1})+1, d(1-1/2^{i})]$. For the edge case $i=(\log d) + 1$, let $W_i$ consist of only the last row of $WF_S$. For convenience, let $\mathcal{R}_i$ denote the index set of rows corresponding to $W_i$, and let $r_i = |\mathcal{R}_i|$ denote the number of rows in $W_i$. Note also that $r_i \leq \frac{d}{2^i}$ for $i \in [\log d]$, and $r_{\log d + 1} = 1$. 
\end{definition}
Then we can write $WF_S$ as $WF_S = [(W_1F_S)^{T};\ldots; (W_{\log d +1}F_S)^{T}]^{T}$. Now consider any $i\in [\log d +1]$ and $W_i F_S$. Since $W_i$ is diagonal and $d/2^{i-1}\leq (W_{i})_{j,j}^2 \leq 2d/2^{i-1}$ for all $j\in [r_i]$, applying Lemma \ref{levscore_reweight} with $\beta = 2\alpha = 2d/2^{i}$ we get the following for all $i\in [\log d + 1]$:
\begin{equation*}
	\tau_{j}(W_i F_S) \leq 2 \tau_{j}(F_{S,i}) \quad \forall j\in [r_i]
\end{equation*}
Here, $F_{S,i}\in \mathbb{C}^{r_i\times s}$ is the matrix consisting of all rows of $F_{S}$ in the index set $\mathcal{R}_i$. %$d(1-1/2^{i-1})+1$ to the $d(1-1/2^{i})$ row.
 Note that the column span of $F_{S,i}$ and the first $r_i$ rows of $F_S$ is identical. This is because the $j^{th}$ column of $F_{S,i}$ is %just $e^{2\pi i (d(1-1/2^{i-1})f_j)}$, which is 
 a constant times the $j^{th}$ column of the matrix formed by considering the first $r_i$ rows of $F_S$. Since the first $r_i$ rows of $F_S$ forms a $r_i \times r$ Fourier matrix, their leverage scores are then identical as well. Finally, we appeal to Corollary C.2 of \cite{eldar2020toeplitz}, restated below:
\begin{corollary}[Corollary C.2 of \cite{eldar2020toeplitz}]\label{corr:C2_eldar}
	For any positive integers $d$ and $s \leq d$, there is an explicit set of values $\wt{\tau}_1^{(s)},\dots,\wt{\tau}_d^{(s)} \in (0,1])$ such that, for any Fourier matrix $F_S \in \mathbb{C}^{d \times s}$ with leverage scores $\tau_1,\dots,\tau_d$,
	\begin{align*}
		&\forall j, \wt{\tau}_j^{(s)} \geq \tau_j \\
		& \sum_{j=1}^d \wt{\tau}_j^{(s)} = O(s \log s)
	\end{align*}
\end{corollary}

Thus by Corollary \ref{corr:C2_eldar} (C.2 of \cite{eldar2020toeplitz}), we easily obtain the following claim.
\begin{claim}\label{levscore_upperbound}
For any $i\in [\log (d/r)]$ and any $j\in [r_i]$ define $\wt{\tau}_{j,i}$ as follows.
\begin{equation*}
\wt{\tau}_{j,i} = \min\left(1,\frac{r}{\min(j,d/2^i+1-j)},\frac{O(r^6\log^3 (r+1))}{(d/2^i)}\right)
\end{equation*}
For any $\log(d/r)<i\leq \log(d)$ and $j\in [r_i]$ let $\wt{\tau}_{j,i}=1$. Then we have the following.
\begin{enumerate}
	\item $\tau_j(W_iF_S) \leq \wt{\tau}_{j,i}$ for all $i\in [\log d]$ and $j\in [r_i]$.
	\item $\sum_{j=1}^{d/2^i} \wt{\tau}_{j} \leq O(r\log r)$ for all $i\in [\log d]$.
\end{enumerate}
\end{claim}
Now we can easily finish the proof of Lemma \ref{leveragescorebound}.
\begin{proof}[Proof of Lemma \ref{leveragescorebound}]
Define $\wt{\tau}_j$ values for $j\in [d]$ as follows.

\begin{equation}
	\wt{\tau}_{j} = \wt{\tau}_{i,j'}
\end{equation}
where $i,j'$ are chosen such that $d(1-1/2^{i-1})+1 \leq j\leq d(1-1/2^{i})$ and $j = d(1-1/2^{i-1})+1 + j'$, and $\wt{\tau}_{i,j}$ are obtained from Claim \ref{levscore_upperbound}. Finally, using Lemma \ref{levscore_submatrix} we can easily conclude that these upper bounds also serve as upper bounds on the leverage scores of $WF_S$, and by \cref{lemma:lev_score_col_span}, upper bounds on the leverage scores of $WF_SR_S$ as well. This completes the proof of Lemma \ref{leveragescorebound}.
\end{proof}



==> filter_functions.tex <==
\section{Filter functions $H$ and $G$}

We use the exact same function $H$ as in \cite{chen2016fourier}. However, because we work with discrete-time Fourier transform, we need the energy guarantees for the grid rather than full interval.

\begin{lemma}[Lemma 6.6 of \cite{chen2016fourier}] \label{lem:H_discrete_properties}
    Constructed with parameters $s_0, s_1, 0 < s_3 < 1, l > 1, 0 < \delta < 1$, with $l = \Theta(k \log(k / \delta))$, the filter function $(H_t, \wh{H}(f))$ has the following properties:\kstodo{add parameter settings somewhere}
    \begin{align*}
        \textnormal{Property I:}& \quad H_t \in [1 - \delta, 1] \quad \forall t \in Z: |t| \leq (\frac{1}{2} - \frac{2}{s_1}) s_3\\
        \textnormal{Property II:}& \quad H_t \in [0, 1] \quad \forall t \in Z: (\frac{1}{2} - \frac{2}{s_1}) s_3 \leq |t| \leq \frac{1}{2} s_3\\
        \textnormal{Property III:}& \quad H_t \leq s_0 \cdot (s_1(\frac{|t|}{s_3} - \frac{1}{2}) + 2)^{-l} \quad \forall t \in Z: |t| \geq \frac{1}{2} s_3\\
        \textnormal{Property IV:}& \quad \textnormal{supp}(\wh{H}(f)) \subseteq [-\frac{s_1 l}{2 s_3}, \frac{s_1 l}{2 s_3}]\\
    \end{align*}
    For any exact $k$-Fourier-sparse signal $x^*_t$ we shift the interval $[0, d]$ to $[-1/2, 1/2]$ and consider $x^*_t$ for $t \in D'$, $D' = \{i/d - 1/2\}_{i \in D}$ to be our observation.
    \begin{align*}
        \textnormal{Property V:}& \quad \sum_{t \in \{i/d - 1/2\}_{i \in \Z} \setminus D'} |x^*_t \cdot H_t |^2 \leq \delta \sum_{t \in D'} |x^*_t|^2\\
        \textnormal{Property VI:}& \quad \sum_{t \in D'} |x^*_t \cdot H_t |^2 \in [1 - \eps, 1] \cdot \sum_{t \in D'} |x^*_t|^2\\
    \end{align*}
    for arbitrarily small constant $\eps > 0$.
\end{lemma}
\begin{proof}
    The first four follow directly from Lemma 6.6 of \cite{chen2016fourier}. Note that we would have to use discrete versions of Lemma 5.1 and 5.5 of \cite{chen2016fourier} to prove this. The discrete version of Lemma 5.1 was shown in \cite{eldar2020toeplitz}, and we state it below.
    \begin{lemma}\label{lem:discrete_lem_5.1}
    	$\forall i\in [d]$, $|x^* (i)|^2 \lsim k^6 \log^3(k)(\|x^*\|_d^2/d) $.
    \end{lemma}
	It is also easy to use this bound in place of its continuous analogue in the proof of Lemma 5.5 in \cite{chen2016fourier} to obtain the following.
	\begin{lemma}\label{lem:discrete_lem_5.5}
		$\forall i\in \mathbb{Z}\setminus [d]$, $|x^* (i)|^2 \lsim k^{13} (ki/d)^{2.2 k}(\|x^*\|_d^2/d) $.
	\end{lemma} 
Equipped with these lemmas about the growth behaviour of $x^*(t)$ inside and outside $[d]$, the proof of Lemma \ref{lem:H_discrete_properties} follows identically as compared to the proof of Lemma 6.6 in \cite{chen2016fourier}.
    \mmtodoil{see Corollary C.2 of https://arxiv.org/pdf/1905.05643.pdf. The polynomial of $k$ is worse than in \cite{chen2016fourier}, check that everything still works. }
\end{proof}
\begin{lemma}[Lemma 6.7 of \cite{chen2016fourier}] \label{lem:G_discrete_properties}
	Given $B>1$, $\delta,\alpha >0$, we set $l=O(k\log(\delta/k))$. Then the filter function $(G_t,\wh{G}(f))[B,\alpha,\delta,l]$ satisfies the following properties,
	\begin{align*}
		\textnormal{Property I:}& \quad \wh{G}(f) \in [1 - \delta/k, 1] \quad if |f| \leq (1-\alpha)/2B.
		\\
		\textnormal{Property II:}& \quad \wh{G}(f) \in [0,1] \quad if (1-\alpha)/2B\leq|f| \leq 1/2B.\\
		\textnormal{Property III:}& \quad \wh{G}(f) \in [-\delta/k,\delta/k] \quad if |f| \geq 1/2B.\\
		\textnormal{Property IV:}& \text{supp}(G(t))\subset [\frac{-lB}{\alpha},\frac{lB}{\alpha}]\\
		\textnormal{Property V:}& \max(G(t))\lsim \poly(B,l)
	\end{align*}

\end{lemma}


==> multi_cluster.tex <==
\subsection{Multi-cluster case}\label{subsection:multi_cluster_freq_recovery}

Our proof for the multi-cluster case largely follows that of \cite{chen2016fourier}, but with one key difference. Due to the on-grid sampling constraint, we cannot handle having multiple large frequencies that are further apart than $\frac{1}{B} = \Theta(\frac{1}{k})$ apart. \kstodo{add technical/intuitive explanation why this is the case} Thus, we first consider the case where all frequencies are within $\frac{1}{B}$ of each other in Section \ref{subsubsection:multi_cluster_bounded_freqs}. Then in Section \ref{subsection:multi_cluster_reduce}, we reduce to this case (where all frequencies are close) by filtering the interval $[0,1]$ into $B$ blocks, one at a time and each of width $\frac{1}{B}$, and recovering the frequencies separately for each block. We now formally define a bounded instance.
\begin{definition}[$(\mathcal{I},\delta')$-bounded instance]\label{def:bounded_freq_case}
	Let $\mathcal{I}\subseteq [0,1]$ be an interval of length bounded by $|\mathcal{I}|\leq 1/B$.
	An instance $x(t) = (x^*\cdot H) (t)+ g(t)$, where $x^*(t) = \sum_{j=1}^k v_j e^{2\pi i f_j t}$ and $g(t)$ is noise, is an $(\mathcal{I},\delta')$-bounded instance if $f_j\in \mathcal{I} \quad \forall j\in [k]$ and $\int_{[0,1]\setminus \mathcal{I}}|\wh g (f)|^2 df\leq \delta'$. The noise threshold $\mathcal{N}^2$ is defined as $\mathcal{N}^2 = \delta \int_{[0,1]}|\wh{x^*\cdot H}(f)|^2 df + \frac{1}{d}\int_{\mathcal{I}}|\wh{g}(f)|^2df+ k\delta'/d\epsilon$.\kstodo{define parametrization and noise threshold properly}
\end{definition}

\subsubsection{Reducing from a bounded instance to $\Theta(k)$ one cluster instances}\label{subsubsection:multi_cluster_bounded_freqs}
In this section, we show how to reduce a bounded instance to $\Theta(k)$ clustered instances. We will only be able to recover ``heavy'' frequencies from a bounded instance
% However, it will be necessary to alter $G$ via $\delta \rightarrow \epsilon\delta$ \hl{to check}, i.e. to make $\hat{G}$ closer to finitely supported.


\begin{definition}[Heavy frequency]\label{def:heavy_freq}
$f^*$ is a heavy frequency if it satisfies
\begin{align*}
\int_{I_{f^*}}|\widehat{x^* \cdot H}(f)|^2 df \geq \frac{d \mathcal{N}^2}{k}
\end{align*}
where $I_{f^*} = [f^*-\Delta,f^*+\Delta]$, and is assumed to wrap around modulo 1. % (the interval is modulo 1).
\end{definition}

\hltodoil{We should include diagrams from CKPS of the $G$ function and maybe $G^j$ with $\sigma=1$}

\begin{definition}[Permutation and filtering notation]\label{def:permutation}
    Let $h_{\sigma, b}(f^*)$ map the frequency $f^*$ to an integer bin between $0$ and $B-1$: $$h_{\sigma, b}(f^*) = \text{round}(\frac{B}{2\pi} \cdot (2\pi \sigma(f^*-b)) \mod 2\pi )$$
    Let $G^{(j)}_{\sigma, b}$ be the function which scales, shifts to $j$, permutes, and approximately filters to a width-$\Delta$ bin (via $G$): $$G^{(j)}_{\sigma, b}(t) = \frac{1}{\sigma}G(\frac{t}{\sigma})e^{2\pi i t (j/B - \sigma b)/\sigma}$$
    When necessary, we will make explicit the parameter $\delta$ used in the construction of $G$ and therefore $G^{(j)}_{\sigma, b}$. 

\end{definition}
\begin{definition}
	Let $z^{(j)} = (x^* \cdot H)\ast G^{(j)}_{\sigma,b}$, $g^{(j)} = g\ast G^{(j)}_{\sigma,b}$and $ x^{(j)} = x\ast G^{(j)}_{\sigma,b} = z^{(j)}+ g^{(j)}$.
\end{definition}
With this notation in hand, we now present the main result of this section below, Lemma \ref{lem:on_grid_lemma_7_6}. It modifies Lemma 7.6 of \cite{chen2016fourier} for on-grid samples.
\begin{lemma}[Lemma 7.6 of \cite{chen2016fourier} for on-grid samples]\label{lem:on_grid_lemma_7_6}
    Let $f^*$ be a heavy frequency of the signal $x^*$. Let $\sigma$ be an \textbf{integer} chosen uniformly in $[\frac{1}{200B\Delta}, \frac{1}{100B\Delta}]$ and $b$ chosen uniformly from $[0, \frac{2\pi d}{\Delta \sigma B}]$\kstodo{why this range of $b$ ? does range of $b$ even matter ?}. Setting $j=h_{\sigma, b}(f^*)$, then $x^{(j)}$ is an $(2\sqrt{\epsilon}, 200\Delta)$-one clustered signal around $f^*$. 
\end{lemma}
The proof will follow the same framework as in \cite{chen2016fourier}, with several intermediate definitions and lemmas.

\hltodoil{Could make this its own subsub(sub?)section, proof of Lemma \ref{lem:on_grid_lemma_7_6}, to keep track of the flow of the proof}

\begin{lemma}[Hashing collision probabilities, analog of Claim 6.4 of \cite{chen2016fourier}]\label{lem:on_grid_claim_6_4}
For $\Delta>0$, let $\sigma$ be sampled uniformly at random from the integers in $[\frac{1}{200B\Delta}, \frac{1}{100B\Delta}]$.
\begin{enumerate}
    \item If $200\Delta \leq |f^+-f^-| < \frac{100(B-1)\Delta}{2}$, then $\mathbb{P}[h_{\sigma, b}(f^+) = h_{\sigma, b}(f^-)] = 0$
    \item If $\frac{100(B-1)\Delta}{2} <|f^+-f^-| < \frac{1}{B}$, then $\mathbb{P}[h_{\sigma, b}(f^+) = h_{\sigma, b}(f^-)] \lesssim \frac{1}{B}$
\end{enumerate}
\end{lemma}
\begin{proof}
    \begin{enumerate}
        \item The proof of this case is unchanged when $\sigma$ is restricted to integers. For completeness: if $200\Delta \leq |f^+-f^-| < 100\frac{(B-1)\Delta}{2}$, then $\frac{2\pi}{B} \leq |2\pi\sigma(f^+-b) - 2\pi\sigma(f^--b)| < \frac{4\pi}{100B\Delta} \frac{100(B-1)\Delta}{2} = (1-\frac{1}{B})2\pi$ Thus, the frequency gap is small enough to avoid wraparound collisions (for which the previous quantity would need to lie in $[(1-\frac{1}{B})2\pi,(1+\frac{1}{B})2\pi]$), and collision is impossible. 
        \item %\hl{this gives intuition but has a bug: it doesn't take into account the range of $\sigma$.} 
        For convenience, let $F = |f^+-f^-|$. For a hash collision to occur, $h_{\sigma, b}(f^+) = h_{\sigma, b}(f^-)$, it must be that $2\pi \sigma F \in (s\cdot 2\pi - \frac{2\pi}{2B}, s\cdot 2\pi + \frac{2\pi}{2B})$ for some integer $s$. This condition is equivalent to $\sigma F \in (s - \frac{1}{2B}, s + \frac{1}{2B})$ for some integer $s$.  Note that the range of possible values of $s$ is $\{\lfloor \frac{F}{200B\Delta }\rfloor,\ldots,\lceil \frac{F}{100B\Delta}\rceil \}$.The rest of the proof proceeds by a simple counting argument based on lengths of intervals. Assume $F < \frac{1}{B}$. 
        %\hl{add floor/ceiling and justify that bounds make sense [eg non-neg] because $F$ is small.}
         For any integer $s$, there are at most $\frac{1/B}{F}+1=\frac{1}{BF}+1$ integer values of $\sigma$ such that $\sigma F \in (s - \frac{1}{2B}, s + \frac{1}{2B})$. Taking into account the total number of possible values of $s$, we get that the total number of such integer values $\sigma$ is at most 
        \begin{align*}
        	(\frac{1}{BF}+1)\cdot ( \lceil \frac{F}{100B\Delta}\rceil - \lfloor \frac{F}{200B\Delta }\rfloor +1) &\leq  (\frac{1}{BF}+1) \cdot (\frac{F}{200B\Delta}+2)\\
        	& \lsim \frac{1}{B^2\Delta}.
        \end{align*}
        Moreover, there are at least $\frac{(B-1)/B}{F} = \frac{B-1}{BF}-2$ integer values of $\sigma$ such that $s + \frac{1}{2B} < \sigma F < (s+1) - \frac{1}{2B}$, i.e. such that $\sigma F$ lies in between this interval and the next one. Again, taking into account the total possible values of $s$ we get that the total number of such integer $\sigma$ is at least
        \begin{align*}
        	(\frac{B-1}{BF}-2)\cdot ( \lceil \frac{F}{100B\Delta}\rceil - \lfloor \frac{F}{200B\Delta }\rfloor -3)
        	&\gsim (\frac{B-1}{BF})\cdot(\frac{F}{100B\Delta})\\
        	&\gsim \frac{1}{B\Delta}
        \end{align*}
        Note that using the notation $\lsim$ and $\gsim$ is justified as $\frac{1}{BF}$ and $\frac{F}{100B\Delta}$ are stricly larger than $1$. Thus we can upper bound the collision probability upto constants by $\frac{1/B^2\Delta}{1/B\Delta}=\frac{1}{B}$.
    \end{enumerate}
\end{proof}

\begin{definition}[Well-isolated frequency, from \cite{chen2016fourier}]
    $f^*$ is well-isolated under the hashing $(\sigma, b)$ if, for j=$h_{\sigma, b}(f^*)$, the signal $\wh{z}^j $ satisfies 
    $$ \int_{[0,1]\backslash (f^*-200\Delta, f^*+200\Delta)} |\wh{z}^{(j)}(f)|^2df \lesssim \epsilon d \mathcal{N}^2/k.$$
\end{definition}

\begin{lemma}[Lemma 7.19 of \cite{chen2016fourier} for on-grid samples]\label{lem:on_grid_7_19_well_isolated} 
Let $f^*$ be any frequency. %, and assume that for any other frequency $f'$ in $x^*$, $|f^*-f'| > \frac{B\Delta}{2}$ implies that the magnitude of $f'$ in $x^*$ is at most $\mathcal{M}$. 
 Then, $f^*$ is well-isolated by a hashing $(\sigma,b)$ with probability $\geq 0.9$ given $B=\Theta(k)$ and $\sigma$ chosen uniformly at random from the integers in the interval $[\frac{1}{200B\Delta}, \frac{1}{100B\Delta}]$ and $b$ is a random real number. \hltodo{Specify how $b$ is chosen} Moreover,
 \begin{equation*}
 	\int_{f^* -200\Delta}^{f^* +200\Delta} |\wh z^{j}(f)|^2 df \gsim \int_{f^*-\Delta}^{f^*+\Delta} |\wh{x^*\cdot H}(f)|^2 df.
 \end{equation*}
\end{lemma}

\begin{proof}
    Let $f^*$ be any frequency, and let $f'$ be another frequency in $x^*$. We divide by cases and draw on Lemma \ref{lem:on_grid_claim_6_4}:
    \begin{itemize}
        \item Due to the random shift $b$ and the fact that the width of the region where $\wh{G}^{(j)}_{\sigma,b}\in [1-\epsilon \delta/k,1]$ is at least $(100-o(1))\Delta$, the entire interval $f^* \pm \Delta$ lands in the same bucket as $f^*$ and in this region of the filter $\wh G^{(j)}_{\sigma,b}$ with probability $0.99$ .
        \item If $200\Delta \leq |f'-f^*| < \frac{1}{\sigma} $, then $\frac{1}{B} \leq |\sigma (f^*-f')|\leq 1 $  implies that the two frequencies are always mapped to different buckets. As a result, they are at distance greater than $\frac{1}{B}$, and fall in the $\frac{\epsilon \delta}{k}$-valued tail of $\wh{G}$. Any such $f'$ contributes at most $\frac{\epsilon \delta}{k} \int_{f'-\Delta}^{f'+\Delta} |\wh{x^* \cdot H}(f)|^2 df$ to the energy in Fourier domain, and thus the total contribution of all such $f'$ is at most $\frac{\epsilon \delta}{k} \int|\wh{x^* \cdot H}(f)|^2 df \leq \epsilon d \mathcal{N}^2/k$ to the energy in Fourier domain.
        \item If $\frac{1}{\sigma} \leq |f'-f^*| \leq \frac{1}{B}$, then by Lemma \ref{lem:on_grid_claim_6_4}, the probability of a hash collision is at most $\frac{1}{B}$, and by taking a union bound over the at most $k$ such $f'$ in the spectrum of $\wh{x^*}$, we have that no such $f'$ lands in the same bucket as $f^*$ with probability at least 0.9. Thus, for any such $f'$, the entire interval $f'\pm \Delta$ again falls in the $\frac{\epsilon \delta}{k}$-valued tail of $\hat{G}$. This implies the total contribution from all such $f'$ to the energy in the Fourier domain is at most $\frac{\epsilon \delta}{k} \int|\widehat{x^* \cdot H}(f)|^2 df \leq \epsilon d \mathcal{N}^2/k$. 
    \end{itemize}
Points 2 and 3 imply that $f^*$ is well-isolated. Point 1 implies that 
 \begin{equation*}
	\int_{f^* -200\Delta}^{f^* +200\Delta} |\wh z^{j}(f)|^2 df \gsim \int_{f^*-\Delta}^{f^*+\Delta} |\wh{x^*\cdot H}(f)|^2 df.
\end{equation*}
\end{proof}
Then the next lemma we need shows that even after multiplying with $\wh{G}^{(j)}_{\sigma,b}$, the signal's energy in the time domain remains concentrated on $[0,d]$.
\begin{lemma}\label{lem:concentrated_in_time}
	Let $f^*$ be any frequency satisfying $\int_{f^*-\Delta}^{f^*+\Delta} |\wh{x^*\cdot H}(f)|^2 \gsim d\mathcal{N}^2/k$. Then $z^{(j)} (t)$ satisfies
	\begin{align*}
		\sum_{t=-\infty}^{\infty}|z^{(j)}(t)|^2 &\gsim  d\mathcal{N}^2/k \\
		\sum_{t\in [-\infty,0]\cup [d,\infty]}|z^{(j)}(t)|^2 dt  &\lsim  \epsilon d\mathcal{N}^2/k.
	\end{align*}
\end{lemma}
The proof of this lemma is identical to the proof of Lemma 7.20 in \cite{chen2016fourier}.
With these tools in place, we are ready to prove Lemma \ref{lem:on_grid_lemma_7_6}.
\begin{proof}[Proof of Lemma \ref{lem:on_grid_lemma_7_6}]
	Let $j = h_{\sigma,b}(f^*)$ and recall $z^{(j)} = x^*\cdot H \ast G^{(j)}_{\sigma,b}$ and $x^{(j)} = (x^* + g)\cdot H \ast G^{j}_{\sigma,b}$. Let $I_{f^*} = [f^*-200\Delta,f^* + 200\Delta]$. Then from Lemma \ref{lem:on_grid_7_19_well_isolated} we know that with probability at least 0.9 the following holds
	\begin{equation*}
		\int_{I_{f^*}} |\wh{z}^{(j)}(f)|^2 df \gsim d\mathcal{N}^2/k,
	\end{equation*}
and the following as well
\begin{equation*}
	\int_{[0,1]\setminus I_{f^*}} |\wh{z}^{(j)}(f)|^2 df \lsim \epsilon d\mathcal{N}^2/k.
\end{equation*}
	Now recall $\wh {g}^{(j)} = \wh{g} \cdot \wh{G}^{j}_{\sigma,b}$.  We need to bound $\int_{[0,1]\setminus I_{f^*}}|\wh{g}^{(j)}(f)|^2 df$. We first bound its expectation as follows.
	\begin{align*}
		\mathbb{E}_{\sigma,b}\left[\int_{[0,1]\setminus I_{f^*}}|\wh{g}^{(j)}(f)|^2 df\right] &= 	\int_{[f^*-1/B,f^*-200\Delta]\cup [f^*+200\Delta,f^*+1/B]}\mathbb{E}_{\sigma,b}[|\wh{g}^{(j)}(f)|^2 ]df  \\
		&+	\mathbb{E}_{\sigma,b}\left[\int_{[0,1]\setminus [f^*-1/B,f^*+1/B]}|\wh{g}^{(j)}(f)|^2 df\right]
	\end{align*}
We assume $supp(\wh{x^*\cdot H}(f))\cap supp(\wh{g}^{(j)}(f))=\emptyset$, otherwise we include the noise in the signal. Using Lemma \ref{lem:on_grid_claim_6_4}, i.e. the probability of collision is upper bounded by $1/B$ for any $f\in[f^*-1/B,f^*-200\Delta]\cup [f^*+200\Delta,f^*+1/B]$. Thus we can upper bound the first term by $\frac{1}{B}\int_{0}^{1} |\wh{g}(f)|^2 df\leq \epsilon d\mathcal{N}^2/k$. To bound the second term we use the fact that the instance is bounded, implying that the energy of the noise outside $[f^*-1/B,f^*+1/B]$ is at most $\delta' \leq \epsilon d \mathcal{N}^2/k$. Thus we finally get the following bound
\begin{equation*}
	\mathbb{E}_{\sigma,b}\left[\int_{[0,1]}|\wh{g}^{(j)}(f)|^2 df\right] \lsim \epsilon d \mathcal{N}^2 /k.
\end{equation*}
Applying markov's inequality we get that with probability at least 0.9, $\int_{[0,1]}|\wh{g}^{(j)}(f)|^2 df \lsim \epsilon d\mathcal{N}^2/k$. Then the previous discussion implies the following
\begin{align*}
	\int_{I_{f^*}}\wh{x}^{j}(f)|^2 df &\geq \int_{f^*-\Delta}^{f^*+\Delta}|\wh{x}^{j}(f)|^2 df\\
	& \geq \int_{f^*-\Delta}^{f^*+\Delta}|\wh{x^*\cdot H}(f)|^2 df \quad  (supp(\wh{x^*\cdot H}(f))\cap supp(\wh{g}^{(j)}(f))=\emptyset)\\
	&\geq d\mathcal{N}^2/k.
\end{align*}
Furthermore,
\begin{align*}
	\int_{[0,1]\setminus I_{f^*}}|\wh{x}^{j}(f)|^2 df &\leq 2\left(\int_{[0,1]\setminus I_{f^*}}|\wh{x^* \cdot H}\cdot \wh{G}^{(j)}_{\sigma,b}(f)|^2 + |\wh{g}^{(j)}(f)|^2 df\right)\\
	& \leq \delta \int_{[0,1]\setminus I_{f^*}}|\wh{x^*\cdot H}(f)|^2 df + 2\int_{[0,1]\setminus I_{f^*}}|\wh{g}^{(j)}(f)|^2df\\
	&\leq \delta \int_{[0,1]}|\wh{x^*\cdot H}(f)|^2 df + \epsilon d\mathcal{N}^2/k = \delta \|x^*\|_d^2 + \epsilon d \mathcal{N}^2/k\\
	&\lsim \epsilon d\mathcal{N}^2/k
\end{align*}
where in the second inequality we used that fact that $|\wh{G}^{(j)}_{\sigma,b}(f)| \leq \delta $ for $f\in [0,1]\setminus [f^*-200\Delta,f^*+200\Delta]$. Thus we have the following.
\begin{equation}\label{freq_concentrated}
	\int_{f^*-200\Delta}^{f^*+200\Delta} |\wh{x}^{(j)}(f)|^2 df \geq (1-\epsilon) \int_{[0,1]} |\wh{x}^{(j)}(f)|^2 df
\end{equation}

Next, our goal is to show that the $x^{(j)}$'s energy in time domain is concentrated in $[0,d]$. Combining Plancherel's theorem, $\wh{g}^{j}(f)=0$ for $f\in I_{f^*}$ and the fact that the noise is zero outside $[0,d]$ in time domain, we get the following 
\begin{equation*}
\sum_{t=0}^{d}|g^{(j)}(t)|^2 = \sum_{t=-\infty}^{\infty}|g^{(j)}(t)|^2  = \int_{[0,1]\setminus I_{f^*}}|\wh{g}^{(j)}(f)|^2 df\leq \epsilon d \mathcal{N}^2/k,
\end{equation*}
and this holds with probability at least 0.9. Combining this with Lemma \ref{lem:concentrated_in_time}, we have that $\sum_{t=0}^d|g^{(j)}(t)|^2 \leq \epsilon \sum_{t=0}^{d}|z^{(j)}(t)|^2$we have the following
\begin{align*}
	\sum_{t=0}^{d}|x^{(j)}(t)|^2 &\geq \sum_{t=0}^{d} |z^{(j)}(t)|^2 - \sum_{t=0}^{d} |g^{(j)}(t)|^2 - 2\sqrt{\sum_{t=0}^{d}|z^{(j)}(t)||g^{(j)}(t)|}\\
	&\geq \sum_{t=0}^{d} |z^{(j)}(t)|^2 - \sum_{t=0}^{d} |g^{(j)}(t)|^2 - 2\sqrt{(\sum_{t=0}^{d}|z^{(j)}(t)|^2)(\sum_{t=0}^d|g^{(j)}(t)|^2)}\\
	& \geq (1-2\sqrt{\epsilon})\sum_{t=0}^d |z^{(j)}(t)|^2.
\end{align*}
Furthermore we have the following
\begin{align*}
	\sum_{t\in [-\infty,0]\cup [d,\infty]}|x^{(j)}(t)|^2 &= 	\sum_{t\in [-\infty,0]\cup [d,\infty]}|z^{(j)}(t)|^2 \\
	&\lsim \eps d \mathcal{N}^2/k \leq \epsilon \sum_{t=0}^d |z^{(j)}(t)|^2.
\end{align*}
The above two inequalities imply the following
\begin{equation}\label{time_concentrated}
	\sum_{t=0}^d |x^{(j)}(t)|^2 \geq (1-2\sqrt{\epsilon})\sum_{t=-\infty}^{\infty} |x^{(j)}(t)|^2
\end{equation}
Thus, equations \ref{time_concentrated} and \ref{freq_concentrated} imply $x^{(j)}$ is an $(2\sqrt{\epsilon},200\Delta)$-clustered signal around $f^*$ with probability 0.9. 
\end{proof}
\subsubsection{Frequency recovery of bounded instances}
Lemmas \ref{lem:on_grid_lemma_7_6} and \ref{lem:on_grid_lemma_7_17} imply the following lemma via a union bound. \hltodo{Should we write the union bound out explicitly in the final version? Reader has to backtrack a lot to the one-cluster lemma.}
\begin{lemma}\label{lem:const_prob_bounded_recovery}
	Let $x(t) = (x^* \cdot H)(t) +  g(t)$ be an $(\mathcal{I},\delta')$-bounded instance. Let $\mathcal{N}^2=\frac{1}{d}\int_{\mathcal{I}}|\wh{g}(f)|^2df+k\delta'/\epsilon+\delta \int_{[0,1]}|\wh{x^*\cdot H}(f)|^2 df$ be the noise threshold. Then the output of \textsc{OneStage} returns a list of $O(k)$ frequencies $L$ such that for any $f^*$ satisfying $\int_{f^*-\Delta}^{f^*+\Delta} |\wh{x^* \cdot H}(f)|^2 df \geq d\mathcal{N}^2/k$, there exists a $
	\wt{f}\in L$ such that $|f^*-f| \lsim \Delta \sqrt{\Delta d}$ with proability at least 0.9	 .
\end{lemma}
\begin{proof}
	Let $j=h_{\sigma,b}(f^*)$, then Lemma \ref{lem:on_grid_lemma_7_6} implies that $x^{(j)} = (x^*+g)\cdot H \ast G^{(j)}_{\sigma,b}$ is $(\sqrt{\epsilon},200\Delta)$-clustered with probability 0.9. \textsc{OneStage} runs \freqrecovcluster on each of the $B$ instances corresponding to each hash bucket and thus returns a list of $B=\Theta(k)$ frequencies, one corresponding to each hash bucket. Applying Lemma \ref{lem:on_grid_lemma_7_17} to the $j^{th}$ bucket, that is on $x^{(j)}$, implies that we can recover a $f$ such that $|f-f^*|\lsim \Delta \sqrt{\Delta d}$ with probability 0.9.
\end{proof}
The next lemma shows how to boost the success probability.
\begin{lemma}\label{lem:bounded_multicluster_recovery}
	Let $x(t) = (x^* \cdot H)(t) +  g(t)$ be a $(\mathcal{I},\delta')$-bounded instance. Let $\mathcal{N}^2=\frac{1}{d}\int_{\mathcal{I}}|\wh{g}(f)|^2df+k\delta'/\epsilon$ be the noise threshold. Then the output of \textsc{MultipleStages} returns a list of $O(k)$ frequencies $L$ such that with probability $1-2^{-\Omega(k)}$, for any $f^*$ satisfying $\int_{f^*-\Delta}^{f^*+\Delta} |\wh{x^* \cdot H}(f)|^2 df \geq d\mathcal{N}^2/k$, there exists a $
	\wt{f}\in L$ such that $|f^*-f| \lsim \Delta \sqrt{\Delta d}$.
\end{lemma}
\begin{proof}
	The proof is identical to the proof of Theorem 2.6 in \cite{chen2016fourier}.
\end{proof}
\subsubsection{Reducing a general instance to a bounded instance}\label{subsection:multi_cluster_reduce}
Consider a general signal $x(t) = x^*(t) + g(t)$, where $x^* (t) = \sum_{j=1}^k v_je^{2\pi i f_j t}$, $f_j\in [0,1] \: \forall j\in [k]$, and $\|g\|_d^2 \leq c \|x^*\|_d^2$ for some small enough \hltodo{small enough with respect to what problem parameters?} constant $c>0$. In this section we explain the reduction from such a general instance to $B=\Theta(k)$ bounded instances.  To achieve this, we convolve with the filter function $G^{(j)}_{\sigma,b}(t)$ as per Definition \ref{def:permutation} with $\sigma=1$, $b$ chosen randomly. The number of buckets used in the $G$ function \ref{lem:G_discrete_properties} to construct $G^{(j)}_{1,b}(t)$ is $B$ and $\alpha  = 1/\poly(k)$. 
To state the main claim of this section, we first need to describe a clustering procedure in Fourier domain (also described in \cite{chen2016fourier}). For any two frequencies $f_1,f_2$ in the support of $\wh {x^*} (f)$ we say that $f_1 \sim f_2$ if their supports overlap after convolving with $\wh H$, i.e. $supp(\wh {H \cdot e^{2\pi i f_1 t}})\cap supp(\wh {H \cdot e^{2\pi i f_2 t}})\neq \emptyset$. We cluster frequencies by taking a transitive closure under this relation $\sim$ and let $C_1,C_2,\ldots, C_l$ denote the clusters. Thus $C_1\cup \ldots \cup C_l = supp(\wh {x^* \cdot H }(f))$ and $C_i \cap C_j = \emptyset$ for any $i \neq j$.  Note that the width of any cluster is at most $k\Delta_H = \poly(k)/d$, here $\Delta_H = |supp(\wh{H}(f))|$.

We now state the main claim of this section below. 
\begin{lemma}\label{lem:gen_to_bounded_reduction}
	Let $z^{(j)}(t) = ((x^*+g)\cdot H) \ast G^{(j)}_{1,b}(t)$, $C_j$ be the union of all clusters landing in bucket $j$ and $S_j$ be the set of all frequencies of $\wh{x^*}(f)$ in $C_j$.  Also $I_j$ is the subset of $[0,1]$ that falls into bucket $j$. Then with probability 0.9, $z^{(j)}(t) = (x^{j}\cdot H)(t) + g^{j}(t)$, where $x^{(j)}(t) = \sum_{f\in S_j} v_f e^{2\pi i f t}$, is a $(I_j,\epsilon \delta d \|x^*\|_d^2/k )$-bounded instance for all $j\in [B]$.
\end{lemma}

 We first make a few important observations about this filtering operation, followed by the proof of the previous lemma.

\begin{claim}
	The hash function $h_{\sigma,b}$ as per Definition \ref{def:permutation} for $\sigma=1$ and $b$ chosen randomly partitions $[0,1]$ into $B$ intervals $[b-1/2B,b+1/2B],[b+1/2B+b+3/2B],\ldots$ where each interval is modulo 1. 
\end{claim}
\begin{claim}[Remark C.15 of \cite{chen2016fourier}]
	Computing $(x\cdot H) \ast G^{(j)}_{1,b}(t)$ for some $t\in [0,d]$ using \textsc{HashToBins} needs the following  samples from $x$ - $x(1-t),x(2-t),\ldots, x(Bl/\alpha-t)$. 
\end{claim}

We now define the notion of a badly cut cluster.
\begin{definition}\label{def:badly_cut_cluster}
	Let $C$ be any cluster as defined above. Suppose there exists a $j$ such that $C\subseteq I_j:=[b+j/2B,b+(j+2)/2B]$. We say that $C$ is ``\emph{not badly cut}'' if $C\subseteq I_j^{inner}:=[b+j/2B + \alpha/2B,b+(j+2)/2B-\alpha/2B]$.
\end{definition}

 Since the width of any cluster is $\poly(k)/d=o(1/B)$, we can show the following Lemma.
\begin{lemma}\label{lem:nothing_badly_cut}
With probability at least $1-o(1)$ over the randomness in $b$, no cluster among $C_1,\ldots, C_l$ is badly cut.
\end{lemma}
\begin{proof}
Since the width of any cluster is at most $\poly(k)/d$ and the width of the good region in any interval is $(1-\alpha)/B = \Theta(1/k)$, the probability that a fixed cluster is badly cut is at most $\poly(k)/d$. Since there are at most $k$ clusters, taking a union bound finishes the proof. 
\end{proof}
We choose a $b$ uniformly at random and condition on the event guaranteed to hold with high probability as per the previous Lemma \ref{lem:nothing_badly_cut}. 

\begin{proof}[Proof of Lemma \ref{lem:gen_to_bounded_reduction}]
Lemma \ref{lem:nothing_badly_cut} combined with the facts that $|G^{(j)}_{1,b}(t)|\leq \epsilon\delta/k$ for all $t\in [0,1]\setminus I_j$ and $|G^{(j)}_{1,b}(t)|\in [1,1-\epsilon \delta/k]$ for all $t\in I_j^{inner}$ from Lemma \ref{lem:G_discrete_properties} implies the following
\begin{align*}
	\int_{[0,1]\setminus I_j}|\wh{z^{(j)}}(f) - \wh{x^{(j)}\cdot H}(f)|^2 df &\leq \frac{\epsilon\delta d}{k} (\int_{0}^{1} |\wh{x^* \cdot H}(f)|^2 df+ \int_{0}^{1} |\wh{g \cdot H}(f)|^2 df)\\
	&\lsim \frac{\epsilon\delta d}{k} \|x^*\|_d^2.
\end{align*}
This implies that $z^{j}(t) = (x^{j}\cdot H)(t) + g^{j}(t)$ is a $(I_j,\epsilon \delta d \|x^*\|_d^2/k)$-bounded instance because the previous equation implies that $\int_{[0,1]\setminus I_j}|\wh{g^{(j)}}(f)|^2 df\lsim \frac{\epsilon\delta d}{k}\|x^*\|_d^2$ and $x^{j}$, an at most $k$-fourier sparse function, has all its frequencies in $I_j$ whose width is $1/B$. 
\end{proof}
\subsection{Sublinear Time Recovery}\label{subsection:sublinear_time_recovery}
In this subsection, our goal is to prove our main theorem , Theorem \ref{thm:sublinear_time_recovery}, which says that we can recover a near optimal low-rank approximation to $T$ in sublinear time. The theorem is formally stated as follows.
We will prove this theorem in few steps. First, we show that if we have noisy access to a symmetric Toeplitz matrix where the noise on the whole matrix has small Frobenius norm, then then noise cannot concentrate on the first half of the first column. 
\begin{lemma}\label{lem:smallnoisefirstcol}
	Let $T$ be a PSD Toeplitz matrix. Suppose $T=\wt T + E$ for some symmetric Toeplitz matrix $\wt T$ such that $\|E\|_F\leq c \|\wt T\|_F$ for some constant $c>0$. Then $\|E_{[:d/2,1]}\|_2\leq 1.98c\|\wt T_{[:d/2,1]}\|_2$.
\end{lemma}
\begin{proof}
	Since $T$ is PSD, we know that 
	\begin{equation}
		\|T\|_F \leq \|T_{[:d/2,:d/2]}\|_F+ \|T_{[d/2:,d/2:]}\|_F.
	\end{equation}
	(add citation for this)
	Since $T$ is also Toeplitz, $T_{[:d/2,:d/2]} = T_{[d/2:,d/2:]}$. Thus we get that $\|T_{[:d/2,:d/2]}\|_F \geq 0.5 \|T\|_F$. Let $T_{on}$ contain only those $d$ diagonals of $T$ defined using entries in $T_{[:d/2,1]}$ and zeros otherwise. Then $\|T_{on}\|_F \geq \|T_{[:d/2,:d/2]}\|_F \geq 0.5 \|T\|_F$. Moreover since each entry of $T_{on}$ is some entry of $T_{[:d/2,1]}$ repeated at most $d$ times, this implies that $\sqrt{d}\|T_{[:d/2,1]}\|_2 \geq \|T_{on}\|_F\geq 0.5 \|T\|_F$. 
	
	Now, note that $\sqrt{d}\|E_{[:d/2,1]}\|_2 \leq \|E\|_F $ (since $E$ is symmetric Toeplitz). Also $\|E\|_F\leq c\|T-E\|_F$ implies $ \|E\|_F \leq 0.99 c \|T\|_F$ by triangle inequality. Thus we have the following.
	\begin{align*}
		\|E_{[:d/2,1]}\|_2 &\leq \|E\|_F /\sqrt{d}\\
		& \leq 0.99c \| T\|_F/\sqrt{d}\\
		& \leq 0.99 c \times  2\sqrt{d} \|T_{[:d/2,1]}\|_2/\sqrt{d}\\
		& = 1.98 c \|T_{[:d/2,1]}\|_2
	\end{align*}
\end{proof}
Next, we present the proof of Lemma \ref{lem:heavy_freq_recovery} we show that we can recover all heavy frequencies of $\wt T$ with high probability.
\begin{lemma}\ref{lem:heavy_freq_recovery}
Fix any $k>0$ and for PSD Toeplitz $T$ let $T = \wt T + E$ with $\wt T = F_{\wt S} \wt D F_{\wt S}^*$ be as guaranteed to exist by Theorem \ref{frobeniusexistence}. Assume $\|E\|_F \leq c\|\wt T\|_F$ for some small enough constant $c>0$. Let $\mathcal{N}^2 = \|E_{[:d/2,1]}\|_2^2 /d + \delta \|\wt T_1\|_{d/2}^2$ be the energy of the noise on the first half of the first column of $T$. Recall $\wt S = \underset{i\in r_1}{\bigcup} S_i$ as per points 2 and 3 of Theorem \ref{frobeniusexistence}. Let $H(t)$ be an approximate rectangle on $[0,d/2]$ as described in Lemma \ref{lem:H_discrete_properties} and $\Delta\geq k \Delta_H=\poly(k)/d$ where $\Delta_H$ is the size of the support of $\wh H$. Then there exists $r_{heavy}\cup r_{light}=[r_1]$ such that the following holds.
\begin{enumerate}
	\item $\wt T^{heavy} = F_{S^{heavy}} D^{heavy}F_{S^{heavy}}^{*}$ where $ S^{heavy} =  \underset{i\in r_{heavy}}{\bigcup} S_i$. Let $L$ be the output of \\ \textsc{k-FrequencyRecovery}, then $|L| = \wt O(k)$ and with probability 0.9, for every $f\in S_{heavy}$ there exists an $\wt f \in L$ such that $|f-\wt f| \leq \Delta \sqrt{\Delta d}$.
	\item $\|\wt T^{light}\|_F \lsim \|E\|_F + \delta \|T\|_F$, where $\wt T^{light} = \wt T - \wt T^{heavy}$.
\end{enumerate}
\end{lemma}
\begin{proof}
Let $x^*(t) = \wt T_1(t)$, a $\wt O(k)$ fourier sparse function, and $g(t) = E_1(t)$. Using Lemma \ref{lem:smallnoisefirstcol} we have that $\|E_1\|_{d/2}^2 \leq 2c\|\wt T_1\|_{d/2}^2$. Let $B =\wt  \Theta(k)$. Now applying Lemma \ref{lem:gen_to_bounded_reduction} we get $B=\wt \Theta(k)$ bounded instances. We apply Lemma \ref{lem:bounded_multicluster_recovery} to each of the bounded instances. Taking a union bound over the randomness in $b$ to ensure Lemma \ref{lem:gen_to_bounded_reduction} and over all bounded instances we can simulatenously recover the heavy clusters from each bounded instance with probability at least $0.9$. We need to bound the energy of the clusters that wont be recoverable from each bounded instance. Consider the bounded instance corresponding to bin $j$ as per Lemma \ref{lem:gen_to_bounded_reduction}. Then the energy of the noise in that instance is 
\begin{align*}
	\mathcal{N}_j^2 &= \frac{1}{d}\int_{ I_{j}} |\wh{g}^{(j)}(f)|^2 df + \frac{\epsilon\delta}{k}\|x^{*}\|_d^2 + \frac{\delta}{d} \int_{[0,1]}|\wh{z^{(j)}}(f)|^2 df\\
	&\leq \frac{1}{d}\int_{ I_{j}} |\wh{g\cdot H}(f)|^2 df + \frac{\epsilon\delta}{k}\|x^{*}\|_d^2 + \frac{\delta}{d} \int_{C_j}|\wh{x^*\cdot H}(f)|^2 df
\end{align*}
where in the second and third inequality we used the fact that $|\wh{g^{(j)}}(f) |= |\wh{g\cdot H} \cdot \wh{G^{(j)}_{1,b}}(f)| \leq |\wh{g\cdot H}(f) |$ for all $f\in I_j$. 
Let $k_j= |S_j|\leq k$ be the number of frequencies in $x^{(j)}$. Then we know that any cluster in $C\in C_j$ satisfying
\begin{equation*}
\int_{C}|\wh{x^{j}\cdot H}(f)| \leq d\mathcal{N}_j^2/k_j
\end{equation*}
has no guarantee of being recovered. However there are at most $k_j$ such ``light'' clusters, and they are disjoint (in fourier domain). Thus the total amount of energy they contribute is at most $k_j\times d\mathcal{N}_j^2/k_j= d\mathcal{N}_j^2$. Moreover light clusters in different bins are disjoint as well. Thus the total amount of energy of light clusters across all bins is at most 
\begin{align*}
	\sum_{j} d \mathcal{N}_j^2 &\leq \sum_j \int_{ I_{j}} |\wh{g\cdot H}(f)|^2 df + \frac{\epsilon\delta}{k}\|x^{*}\|_d^2 + \delta \int_{C_j}|\wh{x^*\cdot H}(f)|^2 df\\
	& \leq \int_{\underset{j}{\cup} I_j}|\wh{g \cdot H}(f)|^2 df + \delta \|x^*\|_d^2\\
	& \leq \int_{[0,1]}|\wh{g \cdot H}(f)|^2 df + \delta \|x^*\|_d^2\\
	& = \|g\cdot H\|_d^2 + \delta \|x^*\|_d^2\\
	&\leq \|g\|_d^2 + \delta \|x^*\|_d^2.
\end{align*} 
where we have adjusted $\delta$ to account for polynomial in $d$ factors (this is feasible as the dependence on $\delta$ is only $\log(1/\delta)$) and the fact that $|H(t)|\leq 1$ for all $t\in \mathbb{R}$.  \\

Recalling that $x^*(t)= \wt T_1(t)$ and $g(t) = E_1(t)$, we apply the previous discussion to $\wt T_1(t)$.
Defining $\wt T^{heavy}$ to be the symmetric Toeplitz matrix whose Vandermonde decomposition has all the frequencies of $\wt T_1$ in all the heavy clusters from each bin and the diagonal $D^{heavy}$ has the corresponding values from $\wt D$, $\wt T^{heavy}(t)$ is the $\wt O(k)$-fourier sparse function defining its first column. Then every frequency in $\wt T^{heavy}$ is recoverable using our algorithm. Let $C_{light}$ be the union of all light clusters of $\wt T_1$. Then from the previous discussion we conclude that 
\begin{align}
\|\wt T_1 (t) - \wt T^{heavy}_1(t)\|_{d/2}^2 &\leq 1.001 \int_{[0,1]} |\wh{H\cdot \wt T_1}(f)-\wh{H\cdot\wt T^{heavy}}(f)|^2 df \\
&=1.001 \int_{C_{light}} |\wh{H\cdot \wt T_1}(f)|^2 df \quad \\
	&\leq  \|g\|_{d/2}^2 + \delta \|\wt T_1\|_{d/2}^2\\
	& = \|E_{[:d/2,1]}\|_{2}^2 + \delta \|\wt T_1\|_{d/2}^2\\
	& \leq \|E_{[:d/2,1]}\|_{2}^2 + \delta \|T\|_F^2 \label{heavylightbound1}
\end{align}

Now define the symmetric Toeplitz matrix $\wt T^{light} = \wt T - \wt T^{heavy}$, then it is easy to see that its first column is defined by $\wt T^{light}_1(t)$. Observe that since the width of each set $\wt S_i $ as per point 2 in Theorem \ref{frobeniusexistence} is $\wt O(\gamma) = \wt O(1/2^{\poly \log d)}) = o(\Delta_H)$, each $\wt S_i$ is either completely in $S^{heavy}$ or completely in $\wt S \setminus S^{heavy}$. This implies $\wt T^{light}$ comprises of PSD buckets replaced with their $\wt O(1)$ rank approximations obtained by applying Lemma \ref{clustered_case-mod} to each bucket. Thus we can say there exists a PSD Toeplitz matrix $T^{light}$ (this is the sum of the PSD buckets) satisfying
\begin{equation}\label{heavylightbound2}
	\|\wt T^{light} - T^{light}\|_F \leq \delta \|T\|_F.
\end{equation} 
Combining equations \ref{heavylightbound1} and \ref{heavylightbound2} and applying triangle inequality we get the following.
\begin{equation*}
	\|T^{light}_{[:d/2,1]}\|_2^2 \lsim \|E_{[:d/2,1]}\|_2^2 + \delta \|T\|_F^2
\end{equation*}
Note that here by adjusting $\delta$ by polynomial factors we have upper bounded $\delta \|\wt T_1\|_{d/2}^2$ in $\mathcal{N}^2$ by $\delta \|T\|_F^2$. Since $T^{light}$ is a Toeplitz matrix, each entry in $T^{light}_{[:d/2,1]}$ appears at most $2d$ times in $T^{light}_{[:d/2,:d/2]}$. Thus we have the following
\begin{align*}
	\|T^{light}_{[:d/2,:d/2]}\|_F^2 &\lsim d\|E_{[:d/2,1]}\|_2^2 + \delta \|T\|_F^2\\
	& \lsim \|E\|_F^2 + \delta \|T\|_F^2  
\end{align*}
where the last inequality follows by observing that since $E$ is also Toeplitz, each entry in $E_{[:d/2,1]}$ appears at most $2d$ times in $E$. Now, since $T^{light}$ is PSD and Toeplitz, we have the following from \cite{audenaert2006norm}
\begin{align*}
	\|T^{light}\|_F &\leq \|T^{light}_{:d/2,:d/2}\|_F+\|T^{light}_{d/2:d,d/2:d}\|_F\\ &\leq 2\|T^{light}_{[:d/2,:d/2]}\|_F.
\end{align*}
Thus we finally obtain that
\begin{equation*}
	\|T^{light}\|_F \lsim \|E\|_F + \delta \|T\|_F.
\end{equation*}
\end{proof}
Now we state the proof of the main theorem, Theorem \ref{thm:sublinear_time_recovery}.
\begin{proof}[Proof of Theorem \ref{thm:sublinear_time_recovery}]
	Recover approx freqs, setup weighted regression problem with these freqs, solve using lev score sampling...
\end{proof}


==> single_cluster.tex <==
\section{Sublinear Time Low-Rank Approximation}
This section of the paper is dedicated to presenting a algorithm for rank-$k$ approximation that has $\poly(k,\log (1/\delta))$ time and sample complexity. It is an adaptation of \cite{chen2016fourier} for discrete-time setting. The main idea is to think about the problem as a sparse Fourier transform of a function $x:\{0, \ldots, d-1\} \to \mathbb{C}$ that is $k$-sparse in Fourier domain, where the access to the function in time is provided only on bounded grid, while the frequencies might be offgrid. To our knowledge, this particular setting was not considered in the literature before, although several works are closely related.
\mmtodoil{elaborate, also elaborate on connection with Frobenius decomposition, add citations}
The main theorem of this section is as follows.
\begin{theorem}\label{thm:sublinear_time_recovery}
	Given any PSD Toeplitz $T\in \mathbb{R}^{d\times d}$, integer $k$ satisfying $k\leq d^c$ for some small constant $c>0$ and parameter $\delta>0$, algorithm \textsc{SublinearTimeRecovery} returns a symmetric Toeplitz $\wt T$ of rank $\poly(k,\log(1/\delta))$ in time $\poly(k,\log(1/\delta))$ such that with probability at least 0.9,
	\begin{equation*}
		\|T-\wt T\|_F \lsim \|T-T_k\|_F + \delta \|T\|_F.
	\end{equation*}
where $T_k = \argmin_{B: rk(B)\leq k}\|T-B\|_F$ is the best rank-$k$ approximation to $T$ in the Frobenius norm.
\end{theorem}

To prove this theorem we first adapt the off-grid frequency recovery algorithm of \cite{chen2016fourier} to the discrete time setting and apply it to the first half of the first column of $T$ \kstodo{explain why first half of first col}. 
\begin{lemma}\label{lem:heavy_freq_recovery}
	Fix any $k>0$ and for PSD Toeplitz $T$ let $T = \wt T + E$ with $\wt T = F_{\wt S} \wt D F_{\wt S}^*$ be as guaranteed to exist by Theorem \ref{frobeniusexistence}. Assume $\|E\|_F \leq c\|\wt T\|_F$ for some small enough constant $c>0$. Let $\mathcal{N}^2 = \|E_{[:d/2,1]}\|_2^2 /d + \delta \|\wt T_1\|_{d/2}^2$ be the energy of the noise on the first half of the first column of $T$. Recall $\wt S = \underset{i\in r_1}{\bigcup} S_i$ as per points 2 and 3 of Theorem \ref{frobeniusexistence}. Let $H(t)$ be an approximate rectangle on $[0,d/2]$ as described in Lemma \ref{lem:H_discrete_properties} and $\Delta\geq k \Delta_H=\poly(k)/d$ where $\Delta_H$ is the size of the support of $\wh H$. Then there exists $r_{heavy}\cup r_{light}=[r_1]$ such that the following holds.
	\begin{enumerate}
		\item $\wt T^{heavy} = F_{S^{heavy}} D^{heavy}F_{S^{heavy}}^{*}$ where $ S^{heavy} =  \underset{i\in r_{heavy}}{\bigcup} S_i$. Let $L$ be the output of \\ \textsc{k-FrequencyRecovery}, then $|L| = \wt O(k)$ and with probability 0.9, for every $f\in S_{heavy}$ there exists an $\wt f \in L$ such that $|f-\wt f| \leq \Delta \sqrt{\Delta d}$.
		\item $\|\wt T^{light}\|_F \lsim \|E\|_F + \delta \|T\|_F$, where $\wt T^{light} = \wt T - \wt T^{heavy}$.
	\end{enumerate}
\end{lemma}
 To prove Lemma \ref{lem:heavy_freq_recovery}, we think of the first column of $\wt T$ as a $\wt O(k)$ fourier sparse function with off-grid frequencies. Then we extend the off-grid frequency recovery algorithm of \cite{chen2016fourier} to our setting where we only have sample access to the function on the integers in time domain. In Section \ref{subsection:one_cluster} we first consider the case when all frequencies of the fourier sparse function lie in one cluster. Then in Section \ref{subsection:multi_cluster_freq_recovery} we reduce the general case to the one cluster case. Finally we prove Lemma \ref{lem:heavy_freq_recovery} and Theorem \ref{thm:sublinear_time_recovery} in Section \ref{subsection:sublinear_time_recovery}.


\begin{comment}
	content...

We define $D = [d] = \{0, \ldots, d-1\}$, with $|D| = d$. Because we can generalize function $x$ defined on $D$ to and $\mathbb{Z}$ \hltodoil{is this supposed to say to a function defined on $\mathbb{Z}$?}, we introduce notation to distinguish between the relevant norms. 
\begin{definition}[Norms of a function] \hfill
\begin{itemize}
    \item For $x$ defined on $D$, $
        ||x||_{D} := \sqrt{\frac{1}{d}\sum_{i \in [d]} |x(i)|^2}
        $
    \item For $x$ defined on $[0, 1]$, $
        ||x||_2 := \sqrt{\int_{0}^{1} |x(t)|^2 \dif t}
        $
    \item For $x$ defined on $\Z$, $||x||_\Z := \sqrt{\sum_{t \in \Z} |x(t)|^2}$
\end{itemize}
\end{definition}
\end{comment}

\begin{comment}
	content...

We will also need the following claim, which states that the discrete and continuous averages for any Fourier sparse function are within polynomial factors of each other. 
\begin{lemma}\label{lem:discrete_continuous_almost_same}
	Let $x^{*}(t)$ be a $k$-Fourier sparse function, defined on the real line. \hltodoil{What is $||\cdot||_d$? Is this supposed to be $||\cdot||_2$? If defined before, repeat it in the definitions above anyway.} Then the following holds.
	\begin{align}
	\frac{1}{d}\sum_{i=1}^{d} |x^*(i)|^2 &\lsim k^4\log^3(k) \|x^*\|_d^2,\quad \text{ and }	\\
	\|x^*\|_d^2 \leq k^{13} \log^5 (k) & (	\frac{1}{d}\sum_{i=1}^{d} |x^*(i)|^2)
	\end{align}
\end{lemma}
In order to prove this lemma, we will need the following helper lemma from \cite{chen2016fourier}.
\begin{lemma}\label{lem:lev_score_helper}[Claim 5.2 in \cite{chen2016fourier}]
	For any $k$ there exists $m= O(k^2\log k)$ such that for any $k$ Fourier sparse function $x^*(t)$, any $t_0\geq 0$ and $\tau >0$, there always exists $C_1,\ldots, C_m \in \mathbb{C}$ such that $|C_i|\leq 11\quad  \forall i\in [m]$ and $x^* (t_0) = \sum_{j\in [m]}C_j x^* (t_0+j\tau)$. 
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:discrete_continuous_almost_same}]
The first point follows from Lemma 5.1 in \cite{chen2016fourier}, which says that $\forall t\in [0,d], |x^*(t)|^2 \lsim k^4 \log^3 (k) \|x^*\|_d^2$. Taking the average over integers in $[0,d]$ completes the proof. Now to prove the second point in the claim, we will follow the proof strategy of Lemma 5.1. We assume without loss of generality that $\underset{t\in [0,d]}{\argmax}|x^*(t)|^2 = 0$, and we can easily reduce to this case if the maximum is not obtained at $t=0$ as described in the proof of Lemma 5.1 in \cite{chen2016fourier}. Then applying Lemma \ref{lem:lev_score_helper} for $t_0 = 0$ and $\tau=1$ we get the following
	\begin{equation*}
		x^*(0) = \sum_{j\in [m]} C_j x^* (j).
	\end{equation*}
Applying Cauchy-Schwarz we get that
\begin{align*}
	|x^*(0)|^2 &\leq m \sum_{j\in [m]}|C_j|^2 |x^*(j)|^2\\
	& \lsim m \sum_{j\in [m]} |x^*(j)|^2.
\end{align*}
Finally, the leverage score bound for discrete time from Lemma C.1 of \cite{eldar2020toeplitz} says that $|x^*(j)|^2 \lsim k^6 \log^3 (k) (\frac{1}{d}\sum_{j=1}^d |x^*(j)|^2)$ for all $j\in [d]$. Using this fact, we obtain the following:
\begin{align*}
	|x^*(0)|^2 &\lsim m^2 k^6 \log^3 (k) (\frac{1}{d}\sum_{j=1}^d |x^*(j)|^2)\\
	&\lsim k^{13} \log^5 (k) (\frac{1}{d}\sum_{j=1}^d |x^*(j)|^2).
\end{align*}
Since $t=0$ was the point at which $|x^*(t)|$ was maximized, taking the continuous average over $[0,d]$ finishes the proof of the lemma.
\end{proof}

\subsection{Small noise on the whole matrix implies small noise on the first half of the first column}

In this subsection we show that if we have noisy access to a PSD Toeplitz matrix, where the Frobenius norm of the noise is small compared to the Frobenius norm of the matrix, then the $\ell_2$ norm of the first half of the first column of the noise is also small compared to the $\ell_2$ norm of the first half of the first column of the matrix. This is formalized in the lemma below.

\begin{lemma}\label{lem:smallnoisefirstcol}
	Let $T$ be a PSD Toeplitz matrix. Assume $T=\wt T + E$ for some Toeplitz matrix $\wt T$ such that $\|E\|_F\leq c \|\wt T\|_F$ for some small enough constant $c>0$. Then $\|E_{[:d/2,1]}\|_2\leq O(c)\|\wt T_{[:d/2,1]}\|_2$.
\end{lemma}
\begin{proof}
	Since $T$ is PSD, we know that 
	\begin{equation}
		\|T\|_F \leq \|T_{[:d/2,:d/2]}\|_F+ \|T_{[d/2:,d/2:]}\|_F.
	\end{equation}
	(add citation for this)
	Since $T$ is also Toeplitz, $T_{[:d/2,:d/2]} = T_{[d/2:,d/2:]}$. Thus we get that $\|T_{[:d/2,:d/2]}\|_F \geq 0.5 \|T\|_F$. Let $T_{on}$ contain only those $d$ diagonals of $T$ defined using entries in $T_{[:d/2,1]}$ and zeros otherwise. Then $\|T_{on}\|_F \geq \|T_{[:d/2,:d/2]}\|_F \geq 0.5 \|T\|_F$. Moreover since each entry of $T_{on}$ is some entry of $T_{[:d/2,1]}$ repeated at most $d$ times, this implies that $\sqrt{d}\|T_{[:d/2,1]}\|_2 \geq \|T_{on}\|_F\geq 0.5 \|T\|_F$. 
	
	Now, note that $\sqrt{d}\|E_{[:d/2,1]}\|_2 \leq \|E\|_F $ (since $E$ is symmetric Toeplitz). Also $\|E\|_F\leq c\|T-E\|_F$ implies $ \|E\|_F \leq 0.99 c \|T\|_F$ by triangle inequality. Thus we have the following.
	\begin{align*}
		\|E_{[:d/2,1]}\|_2 &\leq \|E\|_F /\sqrt{d}\\
		& \leq 0.99c \| T\|_F/\sqrt{d}\\
		& \leq 0.99 c \times  2\sqrt{d} \|T_{[:d/2,1]}\|_2/\sqrt{d}\\
		& = 1.98 c \|T_{[:d/2,1]}\|_2
	\end{align*}
\end{proof}
\begin{comment}
\subsection{Heavy-Light decomposition}
In this section, we show that we can separate $\wt T$ into a Toeplitz matrices $\wt T^{heavy},\wt T^{light}$ such that every frequency in $\wt T^{heavy}$ is heavy in the sense of \cite{chen2016fourier}, and thus recoverable by running their frequency recovery algorithm, and the frobenious norm of $\wt T^{light}$ is small and can thus be absorbed into the noise. This intuition is formalized in the lemma below.
\begin{lemma}\label{heavylightdecomp}
	Fix any $k>0$ and for PSD Toeplitz $T$ let $T = \wt T + E$ with $\wt T = F_{\wt S} \wt D F_{\wt S}^*$ be as guaranteed to exist by Theorem \ref{frobeniusexistence}. Let $\mathcal{N}^2 = \|E_{[:d/2,1]}\|_2^2 /d + \delta \|\wt T_1\|_{d/2}^2$ be the energy of the noise on the first half of the first column of $T$. Recall $\wt S = \underset{i\in r_1}{\bigcup} S_i$ as per points 2 and 3 of Theorem \ref{frobeniusexistence}. Let $H(t)$ be an approximate rectangle on $[0,d/2]$ as described in Lemma \ref{lem:H_discrete_properties} and $\Delta\geq k \Delta_H=\poly(k)/d$ where $\Delta_H$ is the size of the support of $\wh H$. Then there exists $r_{heavy}\cup r_{light}=[r_1]$ such that the following holds.
	\begin{enumerate}
		\item $\wt T^{heavy} = F_{S^{heavy}} D^{heavy}F_{S^{heavy}}^{*}$ where $ S^{heavy} =  \underset{i\in r_{heavy}}{\bigcup} S_i$ and for every $f\in S_{heavy}$
		\begin{equation*}
			\int_{f-\Delta}^{f+\Delta} |\wh {H\cdot \wt T_1^{heavy}}(f)|^2 df \geq d\mathcal{N}^2/{\wt O (k)}.
		\end{equation*}
		Here $\wt T_1(t):\mathbb{R}\rightarrow \mathbb{R}$ is the continuous Fourier sparse function defining the first column of $\wt T$ and $\wh{H\cdot \wt T_1}(f)$ is the DTFT.
		\item $\|\wt T^{light}\|_F \lsim \|E\|_F + \delta \|T\|_F$, where $\wt T^{light} = \wt T - \wt T^{heavy}$.
	\end{enumerate}
\end{lemma}
\begin{proof}
	Let $\wt T_1 (t)$ denote the $\wt O (k)$ Fourier sparse function defining the first column of $\wt T$. Note that our algorithm will only access the first half of the first column of $T$, thus our $H$ function preserves the energies of Fourier sparse functions on $[0,d/2]$. Consider any frequencies $f_1,f_2$ in the support of $\wh {\wt T_1} (f)$, we say that $f_1 \sim f_2$ if their supports overlap after convolving with $\wh H$, i.e. $supp(\wh {H \cdot e^{2\pi i f_1 t}})\cap supp(\wh {H \cdot e^{2\pi i f_2 t}})\neq \emptyset$. We cluster frequencies by taking a transitive closure under this relation $\sim$ and let $C_1,C_2,\ldots, C_l$ denote the clusters. Thus $C_1\cup \ldots \cup C_l = supp(\wh {H \cdot \wt T_1}(f))$ and $C_i \cap C_j = \emptyset$ for any $i \neq j$.  Note that the width of any cluster is at most $k\Delta_H$. We say that cluster $C_i$ is \emph{heavy} if
	\begin{equation*}
		\int_{C_i} |\wh{ H\cdot \wt T_1 }(f)|^2 df \geq d\mathcal{N}^2/{\wt O(k)}.
	\end{equation*}
	Let $S^{heavy}$ denote the set of frequencies in $\wt S$ that appear in heavy clusters, and $\wt T^{heavy}_1(t)$ be the at most $\wt O(k)$ Fourier sparse function corresponding to the heavy frequencies. This in particular implies the following for any $f\in S^{heavy}$
	\begin{align*}
		\int_{f-\Delta}^{f+\Delta} |\wh{H\cdot \wt T^{heavy}_1}(f)|^2 df &= \int_{f-\Delta}^{f+\Delta} |\wh{H\cdot \wt T_1}(f)|^2 df\\
		& \geq d\mathcal{N}^2 / {\wt O(k)}.
	\end{align*}
	Defining $\wt T^{heavy}$ to be the symmetric Toeplitz matrix whose Vandermonde decomposition has frequencies from $S^{heavy}$ and the diagonal $D^{heavy}$ has the corresponding values from $\wt D$, $\wt T^{heavy}(t)$ is the function defining its first column and we conclude the proof of point 1 stated in the theorem.
	
	Let $\wt T^{light}_1(t) = \wt T_1(t) - \wt T^{heavy}_1(t)$. $\wh{H\cdot \wt T^{light}_1}(f)$ contains only the light clusters of $\wh{H\cdot \wt T_1}(f)$  and those are well separated. Combining this with the fact that the $H$ function preserves the discrete energies of at most $\wt O(k)$ Fourier sparse functions, we have the following 
	\begin{align}
		\| \wt T^{light}_1(t)\|_{[0,d/2]}^2 &= \|\wt T_1 (t) - \wt T^{heavy}_1(t)\|_{[0,d/2]}^2 \\
		&\leq 1.001 \int_{C_{light}} |\wh{H\cdot \wt T_1}(f)|^2 df \label{dft}\\
		&\leq  \wt O(k) \times d \mathcal{N}^2/{\wt O(k)} \\
		& \lsim d\mathcal{N}^2	\label{heavylightbound1}
	\end{align}
	where $C_{light}$ is the union of all the light clusters of $\wh{H\cdot \wt T_1}(f)$ and the second to last upper bound follows from the fact that there are at most $\wt O(k)$ light clusters. 
	%One technicality to note here is that the definition of a heavy or light cluster was in terms of the CFT however equation \ref{dft} above is in terms of the DTFT. However note that since $supp(\wh {H\cdot \wt T_1}(f))\subseteq[-\Delta_H,1+\Delta_H]$ all light clusters of $\wh{H\cdot \wt T_1}$ remain identical in the DTFT as well except at most two of them that are within $\Delta_H$ distance of 1 or 0. These may start overlapping and interacting after getting aliased in DTFT, however the energy of the merged cluster can be at most twice the sum of energies of the individual clusters due to Cauchy Schwarz and thus we only lose a constant factor in equation \ref{dft}. 
	Now define the symmetric Toeplitz matrix $\wt T^{light} = \wt T - \wt T^{heavy}$, then it is easy to see that its first column is defined by $\wt T^{light}_1(t)$. Observe that since the width of each set $\wt S_i $ as per point 2 in Theorem \ref{frobeniusexistence} is $\wt O(\gamma) = \wt O(1/2^{\poly \log d)}) = o(\Delta_H)$, each $\wt S_i$ is either completely in $S^{heavy}$ or completely in $\wt S \setminus S^{heavy}$. This implies $\wt T^{light}$ comprises of PSD buckets replaced with their $\wt O(1)$ rank approximations obtained by applying \ref{clustered_case-mod} to each bucket. Thus we can say there exists a PSD Toeplitz matrix $T^{light}$ (this is the sum of the PSD buckets) satisfying
	\begin{equation}\label{heavylightbound2}
		\|\wt T^{light} - T^{light}\|_F \leq \delta \|T\|_F.
	\end{equation} 
	Combining equations \ref{heavylightbound1} and \ref{heavylightbound2} and applying triangle inequality we get the following.
	\begin{equation*}
		\|T^{light}_{[:d/2,1]}\|_2^2 \lsim \|E_{[:d/2,1]}\|_2^2 + \delta \|T\|_F^2
	\end{equation*}
	Note that here, by using Lemma \ref{lem:discrete_continuous_almost_same} to replace the continuous average with the discrete average and adjusting $\delta$ by polynomial factors and using, we have upper bounded $\delta \|\wt T_1\|_{d/2}^2$ in $\mathcal{N}^2$ by $\delta \|T\|_F^2$. Since $T^{light}$ is a Toeplitz matrix, each entry in $T^{light}_{[:d/2,1]}$ appears at most $2d$ times in $T^{light}_{[:d/2,:d/2]}$. Thus we have the following
	\begin{align*}
		\|T^{light}_{[:d/2,:d/2]}\|_2^2 &\lsim d\|E_{[:d/2,1]}\|_2^2 + \delta \|T\|_F^2\\
		& \lsim \|E\|_F^2 + \delta \|T\|_F^2  
	\end{align*}
	where the last inequality follows by observing that since $E$ is also Toeplitz, each entry in $E_{[:d/2,1]}$ appears at most $2d$ times in $E$. Now, since $T^{light}$ is PSD and Toeplitz, we have the following \cite{audenaert2006norm}
	\begin{equation*}
		\|T^{light}\|_F \leq 2 \|T^{light}_{[:d/2,:d/2]}\|_F.
	\end{equation*}
	Thus we finally obtain that
	\begin{equation*}
		\|T^{light}\|_F \lsim \|E\|_F + \delta \|T\|_F
	\end{equation*}
	which completes the proof of the second point in the Theorem statement.
\end{proof}
\end{comment}
\subsection{One cluster case}\label{subsection:one_cluster}

In this Section, we consider discrete time signals that are \emph{clustered} in Fourier domain. The formal definition of such signals is as follows.

\begin{definition}\label{def:one_clustered_signal}[$(\eps, \Delta)$-one-clustered signal]
	For a $f_0$ from $\{0, 1/d, \ldots, (d - 1) / d \}$, a signal $z(t)$ on $\Z$ is $(\eps, \Delta)$-one-clustered around $f_0$ if 
	\begin{align*}
		\textnormal{ Property I: } & \quad \int_{f_0 - \Delta}^{f_0 + \Delta} |\wh{z}(f)|^2 \dif f \geq  (1 - \eps) \int_{0}^{1} |\wh{z}(f)|^2 \dif f \\
		\textnormal{Property II: } & \quad \|z\|_d^2 = \sum_{t \in [d]} |z_t|^2 \geq  (1 - \eps) \sum_{t \in \Z} |z_t|^2 \\
	\end{align*}
\end{definition}
The main result of this subsection is the following lemma, which says that we can approximately recover the central frequency of the clustered signal in sublinear time only using samples of the function that are ``on the grid'' in time domain.
\begin{lemma}\label{lem:on_grid_lemma_7_17}[Lemmas 7.3, 7.17 of \cite{chen2016fourier}]                                                                
	Let $z$ be a $(\epsilon,\Delta)$-clustered signal around $f_0$ for any $\epsilon$ smaller than a small absolute constant and $\Delta = \poly(k)\log(1/\delta)/d$. Then procedure \freqrecovcluster returns an $\wt f_0$ such that with probability at least $1 - 2^{-\Omega(k)}$,
	\[
	|\wt{f}_0 - f_0| \leq \Delta \sqrt{\Delta T}
	\]
	Moreover, \textsc{FrequencyRecovery1Cluster} has time and sample complexity of $\poly (k,\log(1/\delta))$.
\end{lemma}
\subsubsection{Sampling the signal}

The goal of this section is to present algorithms \getempen{} and \getlegsamp{} and show their correctness, with the final goal being \Cref{lem:getlegsamp_corr}. This section is essentially the same as Section 7.2 from \cite{chen2016fourier}, with  algorithms \getempen{} and \getlegsamp{} being \textsc{GetEmpirical1Energy} and \textsc{GetLegal1Sample} but operating on a discrete time signal, rather than a continuous time one. We refer the reader to \cite{chen2016fourier} for the proofs, since they are the same up to the replacement of notation.

% We assume that $\Delta$ is small enough, $\Delta \leq \frac{\text{poly } r}{d}$.

%Let $I = [f_0 - \Delta, f_0 + \Delta]$, $\bar{I} = \mathbb{R} \setminus I$. We define $\wh{z}^{I}(f) = \wh{z}(f)I[f \in I]$ and $\wh{z}^{\bar{I}}(f) = \wh{z}(f)I[f \in \bar{I}]$ where $I[\ldots]$ is the indicator function. $z^I$ and $z^{\bar{I}}$ defined as their inverse Fourier transforms respectively.



We now present algorithms \getempen and \getlegsamp  and their proofs. They are the same as their counterparts from \cite{chen2016fourier}, except that the signal is only accessed on integer points in $[d]$.

\begin{algorithm}[H]
    \SetAlgoLined
    \KwIn{Query access to $z$ on $[d]$, $d$, $\Delta$}
    $R_{est} \gets  O((d \Delta)^2)$\;
    $z_{emp} \gets 0$\;
    \For{$i \in [R_{est}]$}{
        Choose $\alpha_i \in [d]$ uniformly at random\;
        $z_{emp} \gets z_{emp} + |z(\alpha_i)|^2$\;
    }
    $z_{emp} \gets \sqrt{z_{emp} / R_{est}}$\;
    \KwRet{$z_{emp}$}
    \caption{\getempen$(z, d, \Delta)$}\label{alg:GetEmpiricalEnergy}
\end{algorithm}

\begin{lemma}[Counterpart of Claim 7.11] \label{lem:getempen_est_grid}
    \getempen{}, \Cref{alg:GetEmpiricalEnergy}, takes $O((d \Delta)^2)$ samples to output $z_{emp}$ such that $z_{emp} \in [0.8 ||z||_{grid}, 1.2 ||z||_{grid}]$ with probability at least $0.9$.
\end{lemma}
\begin{proof}
    % First we show that $z_{emp} \in [0.9 ||z||_{grid}, 1.1 ||z||_{grid}]$ with probability at least $0.9$.
    The proof follows that of of Claim 7.11 of \cite{chen2016fourier}.
\end{proof}


\begin{algorithm}[H]
    \SetAlgoLined
    \KwIn{Query access to $z$ on $[d]$, $d$, $\Delta$, $\beta$, $z_{emp}$}
    $R_{repeat} \gets  O((d \Delta)^3)$\;
    $S_{heavy} \gets \emptyset$\;
    \For{$i = 1 \to R_{repeat}$}{
        Choose $\alpha_i \in [d]$ uniformly at random\;
        \If{$|z(\alpha_i)| \geq 0.5 z_{emp}$}{
            $S_{heavy} \gets S_{heavy} \cup \{ i \}$\;
        }
    }
    \For{$i \in S_{heavy}$}{
        $w(i) \gets |z(\alpha_i)|^2 + |z(\alpha_i + \beta)|^2$\;
    }
    Choose $\alpha$ among $\alpha_i$, $i \in S_{heavy}$ with probability $w(i) / \sum_{j \in S_{heavy}} w(j)$\;
    \KwRet{$\alpha$}
    \caption{\getlegsamp$(z, d, \Delta, \beta, z_{emp}$)} \label{alg:GetLegalSample}
\end{algorithm}

\begin{lemma}[Counterpart of Lemma 7.2] \label{lem:getlegsamp_corr}
    For a sufficiently small constant $\eps > 0$, $\Delta > 0$, given $\wh{\beta} = \frac{C_{\beta}}{\Delta \sqrt{\Delta d}}$ and $(\eps, \Delta)$-one-clustered signal around $f_0$, \getlegsamp, \Cref{alg:GetLegalSample}, with any integer $\beta \leq 2 \wh{\beta}$ takes $O((d\Delta)^3)$ samples to output $\alpha \in [d]$ such that $\alpha + \beta \in [d]$ and 
    \[
        |z(\alpha + \beta) - z(\alpha)e^{2\pi i f_0 \beta}| \leq 0.08 (|z(\alpha)| + |z(\alpha + \beta)|)
    \]
    with probability at least $0.6$.
\end{lemma}
\begin{proof}
    The proof follows that of Lemma 7.2 of \cite{chen2016fourier}.
\end{proof}

\subsubsection{Cluster of frequencies times $H$ is a one-cluster signal}

\begin{lemma}\label{lem:z_is_onecluster}
    For any $f_0$, $\Delta' > 0$ and $x^*(t) = \sum_{j = 1}^{k} v_j e^{2 \pi i f_j t}$, $|f_j - f_0| \leq \Delta'$ for all $j \in [k]$, let $x(t) = x^*(t) + g(t)$ be our observable signal with noise $g$ such that $||g||^2_{d} \leq c ||x^*||^2_{d}$ for a sufficiently small constant $c$ and $H(t)$ be the filter function with $\mathrm{supp}(H) = \Delta_h$. Then $z = H \cdot x$ is a $(O(\sqrt{c}, \Delta' + \Delta_h))$-one-clustered signal around $f_0$.
\end{lemma}
\begin{proof}
    The proof is the same as for Lemma 7.4 in \cite{chen2016fourier}. The application of Lemma 6.6 is replaced by \Cref{lem:H_discrete_properties}.
\end{proof}

\subsubsection{Frequency recovery}
The main goal of this subsection is to present the algorithms and their proof that can estimate the frequency of a clustered signal upto some additive error. These algorithms use the primitives presented in the previous sub section.


\begin{algorithm}[H]
    \SetAlgoLined
    \KwIn{Query access to $z$ on $[d]$, $d$, $F$, $\Delta$, $z_{emp}$}
    $t \eqsim \log(FT)$, $t' \gets t / 4$, 
    $D_{max} \eqsim \log_{t'}(FT)$, $R_{loc} \eqsim \log_{1/c}(tc)$ ($c<1/2$ is some constant),
    $L^{(1)} \gets 2 F$\;
    \For{$i = 1 \to D_{max}$}{
        $\Delta l \eqsim 2 F / (t')^{i - 1}$,
        $s \eqsim c$, $\wh{\beta} \gets \frac{ts}{2 \Delta l}$\;
        \eIf{$\wh{\beta}\gsim d / (d \Delta)^{3/2}$}{
            \Break
        }{
            $L^{(i)} \gets \textsc{LocateInner}(z, \Delta, d, \wh{\beta}, z_{emp}, L^{i - 1})$\;
        }
    }
    \KwRet{$L^{(D_{max})}$}
    \caption{\textsc{LocateSignal}$(z, d, F, \Delta, z_{emp}$)}
\end{algorithm}

\begin{algorithm}[H]
    \SetAlgoLined
    \KwIn{Query access to $z$ on $[d]$, $\Delta$, $d$, $\wh{\beta}$, $z_{emp}$, $\wh{L}$, variables from \textsc{LocateSignal}}
    $v_q \gets 0, \forall q \in [t]$\;
    \While{$r = 1 \to R_{loc}$}{
        Choose $\beta \in [0.5 \wh{\beta}, \wh{\beta}] \cap \Z$ uniformly at random\;
        $\gamma \gets \getlegsamp(z, \Delta, d, \beta, z_{emp})$\;
        \For{$i \in [m]$}{
            $s_i \in [\beta (\wh{L} - \Delta l / 2), \beta (\wh{L} + \Delta l / 2)] \cap \Z_+$, 
            $\frac{1}{2 \pi \sigma \beta}\theta_i \gets (\phi(x(\gamma) / x(\gamma + \beta)) + 2 \pi s_i)$\;
            Let $q$ be such that $\theta_i \in \text{region}(q)$\;
            Add a vote to $\text{region}(q)$, $\text{region}(q - 1)$ and $\text{region}(q + 1)$\;
        }
    }   
    $q^* \gets \{q | v_q > \frac{R_{loc}}{2}\}$\;
    \KwRet{$L \gets \textnormal{center of region}(q^*) $}
    \caption{\textsc{LocateInner}$(z, \Delta, d, \wh{\beta}, z_{emp}, \wh{L}$)}
\end{algorithm}

\begin{algorithm}[H]
    \SetAlgoLined
    \KwIn{Query access to $z$ on $[d]$, $d$, $F$, $\Delta$}
    $z_{emp} \gets \getempen(z, d, \Delta)$\;
    \For{$i = 1 \to O(k)$}{
        $L_r \gets \textsc{LocateSignal}(z, d, F, \Delta, z_{emp})$
    }
    \KwRet{$L^* \gets \operatorname{median} \{L_r | r \in [O(k)] \}$}
    \caption{\freqrecovcluster$(z, d, F, \Delta$)}
\end{algorithm}

\begin{lemma}[Lemma 7.14 of \cite{chen2016fourier}]
    Let $f_0 \in \textnormal{region}(q')$. Let $\beta$ be sampled uniformly at random from $[\frac{st}{4 \Delta l}, \frac{st}{2 \Delta l}] \cap \Z$ and let $\gamma$ denote the output of procedure \getlegsamp. Then after running the procedure with the pair of samples $z_{\gamma}$, $z_{\gamma + \beta}$
    \begin{itemize}
        \item with probability at least $1 - s$, $v_{q'}$ will increase by one,
        \item for any $|q - q'| > 3$ with probability at least $1 - 15s$ $v_{q}$ will not increase.
    \end{itemize}
\end{lemma}
\begin{proof}
    The proof follows the proof of lemma 7.14 of \cite{chen2016fourier}. The only difference lies in analyzing the case when $|q - q'| > 3$  and $|\theta - \theta_q| \geq \frac{\Delta l}{s t}$. Here, we adopt the analysis of \cite{hassanieh2012nearly} and instead of using Lemma 6.5 of \cite{chen2016fourier}, we will use a corollary of Lemma 4.3 of \cite{hassanieh2012nearly} since our choice of $\beta$ is a random \emph{integer} rather than a random \emph{real number} in some range. 
    
    This Lemma is as follows.
    \begin{lemma}\label{lem:beta_integer}[Corollary of Lemma 4.3 of \cite{hassanieh2012nearly}]
    For some integer number $\wt{m}$, if we sample $\beta$ uniformly at random from a set $\wt{T} \subseteq [\wt{m}]$ of $\wt{t}$ consecutive integers, for any $i \in [d]$ and a set $S \subseteq [d]$ of $\wt{l}$ consecutive integers,
\[
    \Pr[\beta i \mod d \in S] \leq \frac{1}{\wt{t}} + \frac{i \wt{m}}{d \wt{t}} + \frac{\wt{l}\wt{m}}{d \wt{t}} + \frac{\wt{l}}{i\wt{t}}
\]
\end{lemma}
We use Lemma \ref{lem:beta_integer} with the following values ---
    we set $\wt{m} = \lceil \frac{st}{2 \Delta l} \rceil$, 
    $\wt{T} = [\frac{st}{4 \Delta l}, \frac{st}{2 \Delta l}] \cap \Z$, 
    $\wt{t} \geq \frac{st}{4 \Delta l} - 1$, 
    $S = [0, \frac{3s}{4} d ] \cap \Z$, 
    $\wt{l} \leq \frac{3}{4}sd + 1$, 
    $i = d |\theta - \theta_q|$.
Notice that $i$ is in fact an integer, since $\theta = f_0$ is located on a grid with a step $1/d$.
    
Recall that $t = \log d$. By assuming that $d$ is large enough, we assume that $\frac{st}{4 \Delta l} \geq \max(4, 10s^{-1} + 1)$.

    Note that $d \frac{\Delta l}{s t} \leq i \leq d \Delta l$. 
    
    Observe that $\frac{\wt{m}}{\wt{t}} \leq (\frac{st}{2 \Delta l} + 1) / (\frac{st}{4 \Delta l} - 1) \leq 3 $
    
    Hence
    \begin{align*}
        \Pr[\beta i \mod d \in S] & \leq \frac{s}{10} + \frac{3 d\Delta l}{d} + 3 \frac{(3/4) s d + 1}{d} + \frac{(3/4)sd + 1}{d \Delta l (st)^{-1} \cdot (st (4 \Delta l)^{-1} + 1) } \\
        & \leq \frac{s}{10} + \frac{O(1)}{d} + 2s + 9/4 s + 3.1 s \leq 7.5 s
    \end{align*}
	where we used the fact that $\Delta l \leq s/1.5$ since $s= \Theta(1)$ and $\Delta l = o(1)$.

    By the same bound for $S = [-\frac{3s}{4}d, 0]$ and a union bound, we conclude
    \[
        \Pr[\beta d |\theta - \theta_q| \mod d \in [-\frac{3s}{4}d, \frac{3s}{4}d]] \leq 15s
    \]
    which is equivalent to 
    \[
        \Pr[2\pi \beta |\theta - \theta_q| \mod 2 \pi \in [-\frac{3s}{4} 2\pi, \frac{3s}{4} 2\pi]] \leq 15s
    \]
   Thus, overall we get that with probability at least $15s$, $\|2\pi \beta \theta_q - 2\pi \beta \theta\|_\bigcirc > (3s/4) 2\pi $, implying that $v_q$ will not increase.

 \end{proof}
The next lemma essentially gives the final guarantee of the \textsc{Locate1Signal} algorithm.
\begin{lemma}\label{lem:locate1signal_constantprob}[Lemmas 7.15 and 7.16 in \cite{chen2016fourier}]
	The procedure \textsc{Locate1Inner} uses $R_{loc}$ legal samples and then procedure \textsc{Locate1Signal} runs \textsc{Locate1Inner} $D_{max}$ times to output a frequency $\wt{f_0}$ such that $|\wt{f_0} - f_0|\leq \Delta \sqrt{\Delta d}$ with probability at least $0.9$. Moreover, \text{Locate1Signal} has time and sample complexity of $\text{poly}(k,\log(1/\delta))$.
\end{lemma}
\begin{proof}
	The proof is identical to the proofs of Lemmas 7.15 and 7.16 in \cite{chen2016fourier}.
\end{proof}
Finally, the success probability can be boosted by repeating the procedure $O(k)$ times and using the median trick.

\begin{lemma}\ref{lem:on_grid_lemma_7_17}[Lemmas 7.3, 7.17 of \cite{chen2016fourier}]                                                                
	Let $z$ be a $(\epsilon,\Delta)$-clustered signal around $f_0$ for any $\epsilon$ smaller than a small absolute constant and $\Delta = \poly(k)\log(1/\delta)/d$. Then procedure \freqrecovcluster returns an $\wt f_0$ such that with probability at least $1 - 2^{-\Omega(k)}$,
	\[
	|\wt{f}_0 - f_0| \leq \Delta \sqrt{\Delta T}
	\]
	Moreover, \textsc{FrequencyRecovery1Cluster} has time and sample complexity of $\poly (k,\log(1/\delta))$.
\end{lemma}
\begin{proof}
    Follows the proof of original lemma.
\end{proof}
